Rosella: A Self-Driving Distributed Scheduler for Heterogeneous Clusters

Large-scale interactive web services and advanced AI applications make sophisticated decisions in real-time, based on executing a massive amount of computation tasks on thousands of servers. Task schedulers, which often operate in heterogeneous and volatile environments, require high throughput, i.e., scheduling millions of tasks per second, and low latency, i.e., incurring minimal scheduling delays for millisecond-level tasks. Scheduling is further complicated by other users' workloads in a shared system, other background activities, and the diverse hardware configurations inside datacenters. We present Rosella, a new self-driving, distributed approach for task scheduling in heterogeneous clusters. Rosella automatically learns the compute environment and adjusts its scheduling policy in real-time. The solution provides high throughput and low latency simultaneously because it runs in parallel on multiple machines with minimum coordination and only performs simple operations for each scheduling decision. Our learning module monitors total system load and uses the information to dynamically determine optimal estimation strategy for the backends' compute-power. Rosella generalizes power-of-two-choice algorithms to handle heterogeneous workers, reducing the max queue length of O(log n) obtained by prior algorithms to O(log log n). We evaluate Rosella with a variety of workloads on a 32-node AWS cluster. Experimental results show that Rosella significantly reduces task response time, and adapts to environment changes quickly.

==> model.tex <==
\section{Problem formulation and motivation}
\myparab{Modell.} We consider a distributed system that consists of $n$ worker, each of which is connected to a scheduler. The jobs arrive to the scheduler in a streaming fashion. Each job may contain one or more tasks. 
Upon the arrival of a new job, the scheduler can probe a certain number of workers and decides how the tasks should be assigned to the workers based on their queue length. For exposition purpose, our theoretical model focuses on the case where one job contains exactly one task (but our evaluation will consider the general case). 

The jobs are uniform. The arrivals of jobs follow a Poisson distribution with parameter $\lambda$ (\ie the inter-arrival time between two jobs follows an exponential distribution with mean $1/\lambda$). 
Processing power of the workers is heterogeneous. The processing time for a job on worker $i$ follows an exponential distribution with parameter $\lambda_i$. 

For exposition purpose, we assume $\sum_{i \leq n}\lambda_i = 1$ but this requirement is not crucial. On the other hand, we need $\lambda < \sum_{i \leq n}\lambda_i = 1$ to ensure the process is stationary. 

Our goal is to design a simple scheduling algorithm that optimizes one or more of the following metrics: 1. \emph{Expected waiting time.}On average, the amount of time a job waits before it is executed, 2. \emph{Expected completion time.} On average, the amount of time it takes for a job to complete, and 3. \emph{Worst queue length.} At any moment, the length of the longest queue. 

We shall see that expected waiting time and expected completion time are closely related. On the other hand, a bound on the worst queue length ensures that the system is robust and has no outliers from time to time. 

\myparab{Discrete-time counterpart.} 
For analysis purpose, we can couple the continuous time model with a discrete time one using the standard approach. The discrete time model proceeds in rounds. In each round, one of the following events happen 
\begin{itemize}
\item With probability $\lambda/(1+\lambda)$, one new job arrives. 
\item With probability $\lambda_i/(1+\lambda)$, one ``processing'' event happens at worker $i$. This processing event works as follows: if there are one or more jobs exist in the worker's queue, then the oldest job is processed. Otherwise, nothing happens. 
\end{itemize} 
Here, one round in the discrete time process corresponds to a ``jump'' event in the continuous time process. Our major results are stated in terms of the discrete-time system and they can be translated into properties in the continuous-time system in a straightforward manner. 

\subsection{Prior algorithms and their limitation}
In the classical setting, $\lambda_i$'s are assumed to be equal. Below describes two widely used load-balancing algorithms and their key properties.


\myparab{Uniform algorithm.} In this algorithm, upon the arrival of a new job, the scheduler uniformly chooses a worker and put the job over the worker. 

Under this allocation algorithm, the state of each worker follows a Markov chain. Specifically, the Markov chain's state set is the set of non-negative integers. For each time step, the transition probability is as follows: 
\begin{itemize}
\item With probability $(n-1)/n$, the Markov chain remains unchanged. This corresponds to that the event ``hits'' other workers. 
\item With probability $1/n$, the Markov chain will decide to make a move. Conditioned on this event happens, with $1/(2-\epsilon)$ ($\approx \frac 1 2 + \frac{\epsilon}{4}$) probability the Markov chain makes a ``left-move'' (\ie the chain moves to a smaller integer if it is not zero, and stays at $0$ otherwise); with $(1-\epsilon)/(2-\epsilon)$ ($\approx \frac 1 2 - \frac{\epsilon}{4}$) probability that the Markov chain makes a ``right-move''). 
\end{itemize}

Note that in the discrete time model, the Markov chains (workers) are negatively correlated (\ie, if at one specific time step, one worker makes a move, then it implies the rest workers do not move.)

Let $p_i$ be the probabiliy that the chain is at value $i$ at the stationary distribution \Znote{We need to check the actual distribution.}. One can see that $p_i$ decays exponentially \Znote{we may need to compute the exponential decay.} This implies the lemma below.

\begin{lemma}[CITE] Consider the hash-based load balancing algorithm for a system in which $\lambda_i$'s are the same. We have
\begin{itemize}
\item The expected queue length is constant over time. Also, the expected waiting time is constant as well. 
\item With high probability the maximum queue length is $O(\log n)$. 
\end{itemize}
\end{lemma}

\myparab{Power of two choices.} The power-of-two-choices algorithm aims at reducing the maximum queue length over time. The algorithm is also quite straightforward: upon the arrival of a new job, the scheduler probes two random workers and then put the new job to the worker with lighter load. This algorithm is significantly better than the Hash-function based algorithm at the worst case. 

\begin{lemma} [CITE] Consider the power-of-two-choices algorithm for a system in which $\lambda_i$'s are the same, we have whp the largest queue length is $O(\log \log n)$. 
\end{lemma}


 has simple logic and be able to effectively utilize compute resources in the system. We focus on the following three metrics. 

 the scheduler can probe a constant number of workers and then decides which worker should serve for the new job. The jobs are uniform but we assume the arrivals of jobs follow a Poisson distribution with parameter $\lambda$. Processing power of the workers is heterogeneous. For the $i$-th worker, the processing time for a job follows an exponential distribution with parameter $\lambda_i$ (\ie in a unit of time, the worker can process $1/\lambda_i$ jobs on average). 


\mypara{Expected waiting time.} 
\mypara{Expected completion time.} 
\mypara{Worst queue length.} 




Standard coupling argument allows us to have a bijective mapping between events in the continuous time model and those that are in the discrete time model. Thus, for example, the longest queue in the continuous model is the same as the longest queue in the discrete model. 


\section{Motivation}
\Znote{mention that we use P4 switches so that we cannot do
things like late-binding}.


\iffalse
\Znote{Short queue length does not translate into short waiting time.} Notice that even the max queue length for the power of two choices algorithm is $O(\log \log n)$,  the worst waiting time can still be $O(\log n)$ (even when the queue is empty, it could still takes $O(\log n)$ time to process the job). \Znote{so maybe need to ask around why PoT is good.} 

\Znote{Note that in continuous-time model, the queues or machines are independent; but in discrete time model, there 
are some negative correlations among queues.}
\fi

\subsubsection{Failure of these algorithms in heterogeneous system} 
When the compute power of each worker is different, the above algorithms (both the uniform hashing and the power of two choices) fail to work. Below provide two examples illustrating this idea. 

\begin{example} \emph{Uniform hashing does not work.} Consider a system in which there exists 10 workers. The first 9 workers can process one job on average. The last worker can process 2 jobs. So the whole system can on average process 11 jobs in one unit of time. Let the expected number of jobs that arrive in the whole system be 10.5. So we have the processing power of the system is slightly larger than the arrival rate. Now let's see what happens if we use uniform hashing for load balancing. In this case, each of the workers receives 1.05 jobs while these servers can process one job within one time unit. This implies that the process for the regular servers is non-stationary. The length of  queues associated with these servers will be unbounded. 
\end{example}

This problem persists, even using power-of-two-choices. See below for another example. Note here our example needs to use a more skewed system. 

\begin{example} \emph{Power of two choices does not work.} Consider again a system that consists of 10 workers. The first 9 workers can process one job one average. The last worker can process 6 jobs. Let the expected number of jobs that arrive in the whole system be 14. Let us refer to the first nine servers as regular servers and the last server as the fast server. In a power-of-two-choices algorithm, 
with probability $0.9 \times 0.9$ (around 0.81), two regular workers will be selected by the load-balancing algorithm (and the job will go to the one will smaller load). Thus, with probability $0.81$, a new job will go to one of the regular servers. Thus, in one unit of time, on average there are $14 \times 0.81 = 11.34$ jobs that arrive to the collection of regular servers. On the other hand, the total processing power for the regular servers is $9$. So jobs arrive more frequently than the processing power of regular servers. Thus, in long run, the queues associated with the regular servers will ``blow up''. 
\end{example}


\iffalse


\Znote{Copy existing text to here. Also mention that one job maps to one task in this particular work.}
Let $n$ be the total number of jobs in the system. 
We start with considering a continuous time model. The arrivals of jobs follow a Poission distribution, \ie the interarrival time between two jobs follows an exponential distribution with parameter $\lambda$ (so the mean is $1/\lambda$). For each machine, the time to process a job also follows exponential distribution. Different machines have different speed so we let $\lambda_i$ be the paramter for the exponential 
random variable representing the $i$-th worker. The jobs are processed in an FIFO manner. So here $1/\lambda_i$ is the average processing time for the $i$-th worker and $\lambda_i$ is the average number of jobs a worker can process within a unit of them. 
One necessary condition for the system to be stationary (or not ``blow up'') is that the processing power should be a constant fraction larger than the arrival rate. See below for an articulation of this condition.

\myparab{Requirement on the processing power of the distributed system.} Let $\lambda_1$, $\lambda_2$, ..., $\lambda_n$, and $\lambda$ be the variables defined above, a necessary condition for the system to be stationary is 
\begin{equation}
(\lambda_1 + \lambda_2 + ... + \lambda_n) \geq (1+\epsilon) \lambda, 
\end{equation}
where $\epsilon$ is a random variable. 

\textbf{Need to define processing event and how do we couple the continuous time and discrete time process.}
Note that in case the queue of a server is empty, nothing is changed (but there will be a processing event). 
\fi

==> sections/a_analysis.tex <==
\section{Missing proofs}
This section proves Lemma~\ref{lem:loadgood} and Lemma~\ref{lem:l1monotone}. 



\myparab{Conservative estimates:} 
We first show that at the stationary distribution, the marginal distribution of any server decays at least exponentially (at the end, we need doubly exponential decay). Our estimate $\hat \buv_{\pi, i}$ estimates marginal distribution of the load at the $i$-th server, and guarantees that $\Pr[\hat \buv_{\pi, i} \geq j] \geq \Pr[\buv_{\pi, i} \geq j]$ for any $j$. 
 
The conservative estimate comes from a stationary distribution of a coupled process, which we guarantee will dominate the original process. Specifically, let us refer to the original process $\calp$.
The coupled process $\calp_c$ is defined as follows: when a job arrives and we choose two candidate server, we do not place a job only to the shorter queue, we place one job to each of the candidate server (thus we place two jobs in one arrival event). This way of coupling ensures that at any time $\buv_c(t) \prec \buv(t)$, where $\buv_c(t)$ represents the random load vector of $\calp_c$ at time $t$ and $\buv(t)$ represents the random load vector of $\calp$, and $\prec$ represents the component-wise comparison. 

Note that the marginal distributions of $\buv_{c, i}$ (for any $i$) are the same at the stationary distribution (after waiting sufficiently long time). $\buv_{c, i}$ is our estimate $\hat \buv_{\pi, i}$. Note also $\buv_{c, i}$'s (for different $i$) are \emph{not} independent (even we consider the continuous time process). 
The loads of the queues in $\calp_c$ are positively correlated (because the jobs always arrive in bulks). 

We next show that the the tail of $\buv_{c}$ is small, \ie for any suitably small constant $\epsilon$, there exists an $C(\epsilon)$ so that with probability at least $(1-\epsilon)$, at least $(1-\epsilon)$-portion of the nodes are less than $C(\epsilon)$. Here, $C(\epsilon)$ highlights the fact that $C$ depends only on $\epsilon$. 


Because $\buv_c(t) \succ \buv(t)$ for all $t$, we need only analyze the probability that $(1-\epsilon)$ portion of the queue has length $\leq C(\epsilon)$. We cannot use Chernoff-type bounds here because the loads of the queues in $\calp_c$ are not independent. Our crucial observation here is that using Markov inequalities suffices to get what we want. 

Specifically, note that the ``marginal behavior'' for each server (\eg $\buv_{c, i}$ for each $i$) is a Markov chain on $\{0, 1, ..., \}$ so that conditioned on there is a move, the left-transition probability is $1$ and the right-transition probability is $2\alpha$. 

Let $\pi_c$ be the stationary distribution of $\bv_{c, i}(t)$. We have $\pi_c$ exponentially decays in $i$. 
Let $\eta$ be that $\sum_{i \leq \eta}(\pi_c)_i \geq 1 - \epsilon^2$. We see that $\eta$ is a constant when $1 -2\rho$ and $\epsilon$ are constants. 

Let $X_i(T)$ be an indicator variable that sets to 1 if and only if at time $T$ ($T$ here should be treated as the mixing time of the chain: it could potentially depend on the size of the system) if and only if the $i$-th server's load is smaller than $\eta$ at time $T$. We note that $\E[X_i] \geq 1 - \epsilon^2$. Thus, 

\begin{equation}
S \triangleq \frac 1 n \sum_{i = 1}^n \E[X_i] \geq 1 - \epsilon^2. 
\end{equation}

We now use a Markov inequality to bound the probability $\Pr[S \leq 1 - \epsilon]$. Let $\tau = \Pr[S\leq 1 - \epsilon]$. We have 
\begin{equation}
1 - \epsilon^2 \leq \E[S] \leq \tau (1-\epsilon) + (1-\epsilon)\cdot 1 \leq 1 - \tau \epsilon. 
\end{equation}
Thus $\tau \epsilon \leq \epsilon^2$, which implies $\tau \leq \epsilon$. 

Therefore, for any $\buv_{\pi} \sim \pi$ (here, we let $\pi$ be the stationary distribution of the PPoT process), we have with probability $\geq 1 - \epsilon$, the number of over-sized server is at most $\epsilon$ (a server is called oversized if its load is at least $\eta$). When this happens, we say $\buv_{\pi}$ is a good event. We have

\begin{equation}
\E[\bD(\buv, \buv_{\pi})] \leq \E[\bD(\buv, \buv_{\pi}) \mid \buv_{\pi}\mbox{ is good}] + n \cdot \epsilon.
\end{equation}

Next, we introduce an intermediate load vector $\buv_b$ (and couple the load vector $\buv_b$ with $\buv_c$).


\myparab{Truncated queue.} At time $t = 0$, we construct $\bv_b$ as follows: first we sample $v$ from the stationary distribution of the PoT. Then we build $\buv_b = \min \{\bv, \eta\}$ (the min operator here is a component-wise one). We have $\buv_b(0) \leq \bv(0)$ (also component-wise). We first show that there is a coupling that ensures that $\buv_b(t) \prec \buv(t)$ for all $t$. Specifically, we have the following Lemma: 

\begin{lemma} Using the notations above, we have $\buv_b(0) \prec \buv(0)$ and $\buv_b(t) \prec \buv(t)$ for all $t$ under the natural coupling. 
\end{lemma}

\begin{proof} This can be proved by induction. The base case clearly holds. Now assume that before time $t$, the statement holds. Then we need to assume that the hypothesis also holds for time $t + 1$. Assume that $i$ and $j$ are the candidate servers at time $t + 1$. We have the following cases: 

\myparab{Case 1.} $\buv_i(t) < \buv_j(t)$. We may consider three subcases: 

\mypara{Case 1a.} $\buv_{b, i}(t) < \buv_{b, j}(t)$. In this case, $i$ will be used for both processes. The dominance condition continues to hold. 

\mypara{Case 1b.} $\buv_{b, i}(t) = \buv_{b, j}(t)$. In this case, the original process will choose $i$ to process the job. The new process could choose either one, depending on the tie-breaking rule. But our observation is that in either case, the dominance condition will continue to work. Specifically, if the new process chooses $i$, then the loads of servers $i$ are increased at the same time. If the new process chooses $j$, we have $\buv_{b, j}(t+1) = \buv_{b, i}(t) + 1$. On the other hand, $\buv_{b, i}(t) \leq \buv_i(t) \leq \buv_j(t) - 1 = \buv_j(t+1) - 1$. Thus, $\buv_{b, j}(t+1) \leq \buv_{j}(t+1)$. 

\mypara{Case 1c.} $\buv_{b, i}(t) > \buv_{b, j}(t)$. In this case, $j$ will be chosen in the new process. We have $\buv_{j}(t+1) = \buv_{j}(t) > \buv_{i}(t) \geq \buv_{b,i}(t) > \buv_{b, j}(t)$. Therefore, $\buv_{j}(t+1) > \buv_{b, j}(t)$ which implies $\buv_{j}(t+1) = \buv_{b, j}(t)$. 

\myparab{Case 2.} $\buv_i(t) = \buv_j(t)$. The analysis is similar to case 1. Here, we also have three subcases: 

\mypara{Case 2a.} $\buv_{b, i}(t) < \buv_{b, j}(t)$. In this case, $i$ will be chosen to serve the job. The dominance relationship still holds for $j$. 
We have $\buv_i(t) = \buv_{j}(t) \geq \buv_{b, j}(t) >  \buv_{b, i}(t)$. Therefore, $\buv_i(t) \geq \buv_{b, i}(t) + 1$, which implies $\buv_i(t + 1) \geq \buv_{b, i}(t + 1)$. 

\mypara{Case 2b.} $\buv_{b, i}(t) = \buv_{b, j}(t)$. In this case, two processes will apply the same rule to break ties. We can also couple the tie-breaking rule so that servers with the same index will be chosen to serve the job. So after this round, the dominance condition will continue to hold. 

\mypara{Case 2c.} This case is symmetric to the case 2a (it is just flipping the symbols $i$ and $j$). 

\myparab{Case 3.} $\buv_i(t) > \buv_j(t)$. This case is identical to case 1 except that the symbols $i$ and $j$ are flipped. 
\end{proof}

Now we can use the same coupling procedure to argue that $\E[\bD(\bv_b(T) - \bv(T))] = \epsilon$: 

\begin{eqnarray*}
& & \E[\bD(\buv_b(T) - \buv(T))] \\
& = & \Pr[\buv(0) \mbox{ good }]\E[\bD(\buv_b(T) - \buv(T))\mid \bv(0) \mbox{ good }]  \\
& & + \Pr[\buv(0) \mbox{ bad }]\E[\bD(\bv_b(T) - \buv(T))\mid \buv(0) \mbox{ bad }]
\end{eqnarray*}


%\input{analysis_full}

\newpage


==> sections/a_details.tex <==

{\color{red} MAYBE NEED REMOVAL.
After explaining the scheduling algorithm in Section~\ref{sec:potalgo}, we give an example to show why the $\llp$ policy may cause all the workers to slow down. }


{\color{blue} Move the models to here:



We aim to design a simple scheduling algorithm that simultaneously optimizes the following metrics: 

\mypara{1. Waiting time.} When a job arrives, how much time does the system need to process the job? We need multiple statistics to properly characterize the waiting time, including (i). \emph{ Expected waiting time.} On average, the amount of time a job waits before it is executed, (ii). \emph{Expected completion time.} On average, the time it takes for a job to complete; and (iii). \emph{Worst queue length.} Length of the longest queue at any given moment.


Expected waiting time and expected completion time are closely related. On the other hand, a bound on the worst queue length gives a bound on the worst case waiting time. 

{\color{blue} ZL: check we indeed report all these statistics in the experiments}

\mypara{2. Learning and recovery time.} When a system starts up, or experiences a shock (many $\mu_i$ changed), the scheduler does not have accurate estimates on $\mu_i$’s. How much time does the system need to re-learn the $\mu_i$'s, and once learned, how much time does the system need to recover (e.g., handling the backlogs produced by the scheduler using inaccurate/old estimates $\mu_i$)?



}

\section{Related works}
On the theory side, online estimation and learning are an extensively studied area~\cite{poor2013introduction}. Stochastic optimization and exponential moving average~\cite{harold1997stochastic} are widely used techniques to estimate means of a sequence of i.i.d. random variables. 

Mention change point detection ~\cite{tartakovsky2014sequential}

\begin{itemize}
\item Dean's 'Tail at scale'. 
\item Adaptive load sharing in homogeneous distributed systems. 
\item Fair Scheduling for Distributed Computing Clusters
\item Mesos, Yarn, Omega, 

\end{itemize}

load balancing algorithms (sometimes under the name ``balls-and-bins'') and power-of-two-choices in homogeneous systems have been extensively studied. 
See~\cite{Mitzenmacher2005} for a comprehensive treatment of balls-and-bins, ~\cite{Mitzenmacher00thepower} for a survey of power-of-two-choices algorithms in discrete-time systems, and~\cite{ying2017power,xie2015power} for more recent development.
 For the continuous-time counterpart, see \eg~\cite{McDiarmid05,Bramson2010} and references therein. 

On the system side, recent works include Omega~\cite{schwarzkopf2013omega}, which addresses the concurrency issues among schedulers. Ananta ~\cite{patel2013ananta} is a layer-4 load-balancer that combines techniques in networking and distributed systems to refactor its functionality to meet scale, performance, and reliability requirements.  Duet~\cite{gandhi2015duet} 
is a distributed hybrid load balancer that fuses switch with the software load balancers. Apollo~\cite{boutin2014apollo} is a coordinated scheduling framework that is suitable of executing ``heavy jobs'' (those require heavy resources). 
Sparrow~\cite{ousterhout2013sparrow} is most related to our work. There, the notion of late binding and batching are introduced and integrated with PoT technique. But Sparrow assumes the system is homogeneous. 


 

\iffalse
To the best or our knowledge, PSS is a novel approach building a 
distributed, sampling-based scheduler in clusters where servers possess heterogenous compute-power. 
There are plenty of distributed load balancers schemes. However, they assume the servers are uniform.  A brief review is 
illustrated below.


There are plenty of distributed load balancers schemes, we just give a brief review.
Sparrow's \cite{ousterhout2013sparrow} uses 
 batch sampling with the power of two choices.  Tasks are scheduled on servers with the shortest queue. 
Such schedulers fail to gain advantage from
heterogeneous clusters where completion time is affected by compute-power.
 Sparrow uses late binding to alleviate its reliance on queue length, however, as shown in our experiments, Sparrow's performance degrades in the heterogenous cluster. 

Omega ~\cite{schwarzkopf2013omega} supports multiple distinct workloads under the architecture using 
parallelism, shared state, and optimistic
concurrency control. Ananta ~\cite{patel2013ananta} is a distributed layer-4 software load balancer while Duet ~\cite{gandhi2015duet} 
is a distributed hybrid load balancer focusing on fuses switch with the software load balancers.
Baraat~\cite{dogar2014decentralized}  is a decentralized system for task-aware network scheduling based on FIFO mechanism for data centers.
Apollo system ~\cite{boutin2014apollo}  uses per-job schedulers
 where various factors holistically and performs estimation- based scheduling is considered to minimize task completion time.
 
\fi


\begin{itemize}
\item Uniform random: 
\item Sparrow without late-binding: The classical power-of-two-choices algorithms. 
\item Sparrow with late-binding:  The full-fledged Sparrow that integrates a so-called “late-binding” technique with POT. 
\item The scheduler for heterogeneous clusters that assumes accurate information on worker speed. 
\item Multi-arm (baseline): 
\item \sysname with one probe (i.e., PSS+Learning): The simplified Rosella algorithm that continuously estimates worker speed and uses the estimates to run proportional sampling algorithms. 
\item \sysname (i.e., PSS+PoT+Learning): The full-fledged Rosella system.
\end{itemize}

==> sections/amodel.tex <==
\myparab{Mappings between discrete time and continuous time.} Because there exists an elegant mapping between continuous time and discrete time, key statistics in the continuous time model can often be mapped to key statistics in the discrete time model. 

\mypara{Comparing between exponential random variables and geometric random variables.} In the continuous time model, the inter-arrival time (between jobs) and processing time of workers follow exponential distribution. In the discrete time model, the inter-arrival time and processing time becomes geometric distribution. Below lists the similarities and differences of exponential and geometric r.v.s: 

%copy down macros I need. 
%\newcommand{\expn}{\mathrm{Exp}} 
%\newcommand{\geom}{\mathrm{Geo}}

\begin{itemize}
\item In continuous time model, the processing time for the $i$-th server is $\expn(\lambda_i)$. The expectation is $1/\lambda_i$. 
\item In discrete time model, the processing time for the $i$-th server is $\geom(\lambda_i/C)$. The expectation is $C/\lambda_i$. 
\end{itemize}
Similar things can be said about the inter-arrival time. We make two observations: 

\begin{itemize}
\item 1 unit of time in the continuous time 
\item the discrete time model is ``scale-invariant'', \ie if we scale $\lambda_i$ and $\lambda$ by a constant, the corresponding discrete-time model remains unchanged. So to simplify our discussion, we make these additional assumptions: (a) $\sum_{i = 1}^n \lambda_i = 1$, and (b) $\lambda = (1-\epsilon)$, to reflect the fact that the system's processing power is a little larger than the jobs' arrival rate. 
\end{itemize}

\Znote{Somehow we need to argue that sometimes discrete and continuous systems are not exactly the same but for practical purpose, they are equivalent.}


\subsection{A brief overview of existing solutions}


\section{Additional questions for MM.} 
\begin{itemize}
\item Is that a solved problem (the landscape is much less clear for heterogenous servers)? 
\item Did MM try such problems before? And what's the reasons that he did not publish anything? 
\end{itemize}


==> sections/analysis.tex <==
\vspace{-3mm}
\section{Analysis of the algorithms}\label{sec:analysis}
\vspace{-3mm}
\myparab{Our model.} 
For simplicity, our theoretical model focuses on the case of one job containing one task (but our evaluation will consider the general case). The arrivals of jobs follows a Poisson distribution with parameter $\lambda$. Processing/compute power of the workers is heterogeneous. The service time for a job assigned to worker $i$ follows an exponential distribution with parameter $\mu_i$. 
Let $\mu = \sum_{i \leq n} \mu_i$ be \emph{the system's the total processing power}, and $\alpha = \lambda / \mu$ be the system's \emph{load ratio}. 
Both $\mu_i$ and $\lambda$ can change over time to reflect volatility in the system. %For simplicity, let the total processing power always be larger than 
$\bar \mu$, which is always larger than the job arrival rate. 

%We consider a distributed system that consists of $n$ workers/servers, each connected to a scheduler. Jobs arriving to the scheduler may contain one or more tasks. When a new job arrives, the scheduler probe a certain number of workers and decide how  to assign tasks based on workers' queue length. 




\vspace{-1mm}
\myparab{Discrete-time counterpart.} 
We use a standard way to couple our continuous time model with a discrete time model~\cite{ross2014introduction}. The discrete time model proceeds in rounds. One of the following events occurs in each round: (i) With probability $\lambda / (\lambda + \mu)$, one new job arrives, and (ii)  With probability $\mu_i / (\lambda + \mu)$, one processing event happens at worker $i$ as follows: if the worker's queue contains one or more jobs, the the oldest job is processed first. Otherwise, nothing happens. 
One round in the discrete time model corresponds to a ``jump'' event in the continuous time model. Since we have coupled models (e.g., a convergence result for one often implies a similar result for the other), our analysis can switch between them to deliver an intuitive analysis.

\vspace{-1mm}
\myparab{Main results.} Our system is highly efficient and scalable: 
\emph{Result 1. Maximum load.} With high probability the maximum queue length is $O(\log \log n)$ at the stationary distribution, generalizing existing PoT results. \emph{Result 2. Learning speed.} The time to learn \emph{all the parameters $\mu_i$} is $O\left(\frac{\log (1/n)}{(1-\alpha)^2}\right)$. Thus, when the number of workers doubles, it takes only a constant amount of additional time to learn the system. 
\emph{Result 3. Convergence time.} When the system has reliable estimates of the processing powers, it takes additional $O(1)$ time to converge to the stationary distribution. 

\iffalse
\begin{figure*}[t!]
 \includegraphics[scale=0.4]{figures/timeline.pdf}
  \centering
  \caption{
  \vspace{-.05cm}Roadmap of our theoretical analysis. At the stationary state $t_1$, the max queue length is $O(\log \log n)$ (Lemma~\ref{lem:loglog}); at time $t_2$, the system experienced a shock so that three workers changed their processing power. It takes $O(\log(1/n)$ time to re-learn the new processing power (time spent from $t_2$ to $t_3$). See Lemma~\ref{lem:learn}. At $t_3$, we learned the parameters but some queues have backlogs (the red one). It takes an additional $O(1)$ amount of time to recover (form $t_3$ to $_4$, Proposition~\ref{prop:mixing}). \color{red} Change figure}
    \label{fig:timeline}
\end{figure*}
\fi

\myparab{Interpreting the results.} 
Consider the ``life cycle'' of \sysname. 
At $t_1$, \sysname is in stationary distribution. We apply result 1: 
the maximum load at $t_1$ is $O(\log \log n)$ with high probability. At $t_2 > t_1$, the system experiences a shock (the processing power of a large number of workers get changed) and the estimates are no longer correct.
\sysname re-learns the new worker speeds. Result 2 states that the learning time is $O(\log 1/n)$. Let $t_3 = t_2 + O(\log 1/n)$ be the time the system re-learns the worker speeds. At this time, there could be backlogs during the learning (between time $t_2$ and $t_3$) since the system has been using inaccurate estimates. Result 3 states that it takes $O(1)$ time to clear up backlogs. 
%So we need to wait more time for \sysname to return to normal.

\vspace{-1mm}
\myparab{Notations.} We use $u, v$ to represent vectors, where $u_i$ ($v_i$) represents the $i$-th entry of $u$ ($v$). $\buv$ and $\bvv$ are random vectors. We refer \sysname as a PPoT process (\textbf{p}roportional sampling + PoT). We denote a PPoT process as $\{\buv(t)\}_t$. Let the stationary distribution of a PPoT be $\buv_{\pi}$. Abusing the notation, let $\{\buv_{\pi}(t)\}$ be a PPoT process that starts with stationary distribution. 
Below, we explain our analysis of the three key results. We start with result 2 because the analysis is more complex, followed by results 1 and 3.

\vspace{-3mm}
\subsection{The ``recovery time'' of the PPoT process}\label{sec:recovery}
\vspace{-3mm}
Assume that \sysname starts with an arbitrary state (\eg recently experienced a shock) and our algorithm knows the exact $\mu_i$'s, Sec.~\ref{sec:recovery} bounds the time needed for a PPoT process to converge to the stationary distribution. 

\vspace{-1mm}
\myparab{Defining recovery time.}
One way to define recovery time is the mixing time, \ie the time for the load distribution to be statistically-close to the stationary distribution, where the statistical distance between two random vectors $\bvv$ and $\buv$ is defined as 
$\|\buv - \bvv\|_{\tv} = \sum_{w} \|\Pr[\buv = w] - \Pr[\bvv = w]\|_1$. The example below shows the statistical distance is an unsuitable metrics. 
\vspace{-1mm}
\begin{example}\label{example:load}\emph{
Consider two systems whose loads are represented by $\buv$ and $\bvv$. Let $\buv_1 = 1$ and $\bvv_1 = 0$ (\ie worker 1 in $\buv$ always has 1 task while it always has 0 task in $\bvv$). The rest workers have i.i.d. distribution. Intuitively, the distributions of two systems should be close because they differ only on the first servers. But $\|\buv - \bvv\|_{\tv}$ is 1 because their supports are disjoint (coming from the fact $\buv_1$ and $\bvv_1$ never agree).
}
\vspace{-5mm}
\end{example}

We use a new metric to better capture the closeness between two systems. 
Recall that the $\ell_0$-distance two vectors is  
$\| u - v\|_0 = \frac 1 n \sum_{i = 1}^n I(u_i \neq v_i)$, where $I(\cdot)$ is an indicator function that sets to one when its argument is true. We have,

\vspace{-1mm}
\begin{definition}[$\ell_0$-distance between loads] The $\ell_0$-distance between two random vectors $\buv$ and $\bvv$, namely $\bD(\buv, \bvv)$, is at most $\epsilon$ if there is a way to couple $\buv$ and $\bvv$ such that 
$\E[\|\buv - \bvv\|_0] \leq \epsilon$.
\vspace{-2mm}
\end{definition}

This definition measures only the number of servers that have different loads in two systems. In Example~\ref{example:load}, the statistical-distance between them is $1$, but the $\ell_0$ distance is $\frac 1 n \rightarrow 0$, as $n$ grows, thus properly capturing the fact that two systems are close.  
%The $\ell_0$-distance captures the notion of ``closeness of load vectors'' well. In the previous example (in which we consider two systems such that $\bvv_1 = 1$ and $\buv_1 = 0$). While 
%Let $\buv_{\pi}(t)$ be the load vector at time $t$ of a PPoT process that starts at the stationary distribution. 
Let $\bvv(t)$ be the load vector at time $t$ of a PPoT process that starts at an arbitrary state with $C_{\max} = \|\bvv(0)\|_{\infty}$. 
\vspace{-1mm}
\begin{definition}[Recovery time] Using the notations above, the recovery time $T(\bvv, \epsilon)$ of a PPoT process that starts with $\bvv$ is 
$
T(\bvv, \epsilon) = \min_t \left\{\bD(\bvv(t), \buv_{\pi}(t)) \leq \epsilon \right\}.$
\vspace{-2mm}
\end{definition}

Intuitively, after $T(\bvv, \epsilon)$ time, only $\epsilon$-portion of the workers are inconsistent with the stationary distribution. The rest workers all recovered. We have
\vspace{-2mm}
\begin{proposition}\label{prop:mixing} Using the notations above, the recovery time $T(\bvv, \epsilon) = O(C_{\max}\log (1/\epsilon))$, \ie it \emph{does not depend} on the size $n$ of the system. 
\vspace{-2mm}
\end{proposition}

For simplicity, we assume that $\alpha$ is suitably small. Techniques developed in our analysis can be generalized for arbitrary $\alpha$. Proving Prop.~\ref{prop:mixing} consists of two major steps: 

\vspace{-1mm}
\myparab{Step 1. A conservative estimate of the stationary distribution.} Let $\{\bvv(t)\}_t$ be an arbitrary PPoT process and $f_i$ be the PDF for the marginal distribution of worker $i$ at the stationary state. The tail of $f_i$ decays with at least exponential rate (\ie $f_i(j) \leq \rho f_i(j+1)$ for some $\rho < 1$) since the PPoT algorithm is at least as good as the proportional sampling algorithm. With Markov inequality, we have:
\vspace{-2mm}
\begin{lemma}\label{lem:loadgood} Let $\epsilon$ be an arbitrary constant and $\buv_{\pi}$ be the stationary distribution. Let $\buv_{\pi, i}$ represent the $i$-th coordinate of $\buv_{\pi}$. There exists a constant $\eta$ (that depends only on $\epsilon$) such that that: $
\Pr\left[\sum_{i \leq n}I(\buv_{\pi, i} \leq \eta) \leq (1-\epsilon) n\right] \geq 1 - \epsilon.$
\end{lemma}
\vspace{-2mm}
Lemma~\ref{lem:loadgood} implies that at the stationary distribution, most workers will have constant queue length. 
We also observe that $\|\bvv(t) - \buv_{\pi}(t)\|_0$ is \emph{not} monotonically decreasing and thus it is remarkably difficult to directly track this quantity. Thus, we focus on the evolution of $\|\bvv(t) - \buv_{\pi}(t)\|_1$:
\vspace{-5mm}
\begin{lemma}\label{lem:l1monotone} Using the notations above, we have $\|\bvv(t) - \buv_{\pi}(t)\|_1 \geq \|\bvv(t) - \buv_{\pi}(t)\|_0$. Moreover, $\|\bvv(t) - \buv_{\pi}(t)\|_1$ is monotonically decreasing regardless of the initial state $\bvv(0)$.  
\vspace{-5mm}
\end{lemma}

The monotone property is a known result and can be proved by a simple combinatorial analysis. See also~\cite{bramson2012asymptotic}. 

\vspace{-1mm}
\myparab{Step 2. $\|\bvv(t) - \buv_{\pi}(t)\|_1$ shrinks quickly.} We next show that $\|\bvv(t) - \buv_{\pi}(t)\|_1$ has exponential decay. 
We need to circumvent two key challenges: \emph{(i)} The discrepancies in loads at the same workers could increase, \ie it is \emph{not true} that $|\bvv_{i}(t) - \buv_{\pi, i}(t)|\leq |\bvv_{i}(t+1) - \buv_{\pi, i}(t+1)|$. 
Therefore, we cannot focus on individual workers only. \emph{(ii)} The loads of different workers are correlated. 

Our key idea is to identify a group of events that occur sufficiently often, and when such an event occurs, $\|\bvv(t) - \buv_{\pi}(t)\|_1$ strictly decreases. 
A deletion event at time $t$ at workers $i$ is a \emph{good deletion event} if worker $i$ is empty in one of $\{\bvv(t), \buv_{\pi}(t)\}$ and non-empty in the other one. A good deletion event has no effect on, for example, $\bvv_i$ but $\buv_{\pi, i}$ is decremented by one. After the deletion, we have $\|\buv_{\pi}(t+1) - \bvv(t+1)\|_1$ is decremented by 1. The frequency of good deletion events is:
%characterized by the following lemma. 
\vspace{-2mm}
\begin{lemma}\label{lem:shrink}Using the above notations, there exists a constant $C$ such that with constant probability, 
$\|\bvv(t+C) - \buv_{\pi}(t+C)\|_1 \leq c_1 \|\buv_{\pi}(t) - \bvv(t)\|_1
$
\vspace{-3mm}
\end{lemma}

\mypara{Outline of the proof.} When the loads of workers $i$ are different in two processes, each loads perform a ``left-drifting random walk'' with a left bound $0$. With a constant probability, within $\Theta(1)$ steps, one walk will hit zero first, and 
a good deletion event will occur. We next need to count the number of workers with different loads at $t$, \ie $\|\bvv(t) - \buv_{pi}(t)\|_0$. We observe that with high probability $\|\bvv(t) - \buv_{\pi}(t)\|_0 = \Theta(\|\bvv(t) - \buv_{\pi}(t)\|_1)$. 
When we have large number of excessively long queues, $\ell_0$-norm of a vector could be much smaller than the $\ell_1$-norm. But having excessive long queue is a rare event; we can use this intuition to show that $\ell_1$-norm and $\ell_1$-norm of  $\bvv(t) - \buv_{\pi}(t)$ are in the same order. 
Lemma~\ref{lem:shrink} and the fact that $\|\bvv(t) - \buv_{\pi}(t)\|_0 = \Theta(\|\bvv(t) - \buv_{\pi}(t)\|_1)$ imply $\|\bvv(t) - \buv_{\pi}(t)\|_0$ shrinks by a constant portion in $O(1)$ time. Prop.~\ref{prop:mixing} the follows. 

\iffalse
We now calculate the recovery time. Let $k = \|\bvv(t_0) - \buv_{\pi}(t_0)\|_1 = O(C_{\max})$ for some $t_0$. Since $\|\bvv(t_0) - \buv_{\pi}(t_0)\|_1 = \Theta(\|\bvv(t_0) - \buv_{\pi}(t_0)\|_0)$, we have $\|\bvv(t_0) - \buv_{\pi}(t_0)\|_0 \geq c_1 k$ for some constant $c_1$. 
After waiting a constant amount of time (say $\Delta$), the number of good deletion events is in the order of $c_1k$. Thus, we have $\|\bvv(t_0 + \Delta) - \buv_{\pi}(t_0 + \Delta )\|_1 \leq (1-\Theta(c_1)) \|\bvv(t_0) - \buv_{\pi}(t_0)\|_1$, which implies that the $\ell_1$-distance shrinks by a constant factor. Thus, it takes $O(C_{\max}\log(1/\epsilon))$ rounds to reach a state such that $\|\bvv - \buv_{\pi}\|_1 \leq \epsilon$. This proves Proposition~\ref{prop:mixing}. 
\fi

\vspace{-3mm}
\subsection{Stationary distribution of a PPoT process}\label{sec:potanalysis}
\vspace{-2mm}
Using the framework developed in~\cite{bramson2010randomized,bramson2012asymptotic}, we analyze the stationary distribution based on an ansatz~\cite{bramson2012asymptotic}:
consider the load balancing system described above that operates under the $\sqq$-policy, with $\alpha < 1$. When $n \rightarrow \infty$, there is a unique equilibrium distribution. Moreover, under this distribution, any finite number of queues are independent.
%~\footnote{Interested readers could also generalize the analysis in to prove the ansatz.}.

Our main result is that the marginal stationary distribution of all the workers is the same, regardless of their processing power. 
Consider the first queue and sample its processing power from a power law distribution. The potential arrival process at queue 1 consists of jobs that have worker 1 as one of the choices.  At any time $t$, let the empirical distribution of queues $2, \dots, n$ be denoted by $\mu^n(t)$, \ie $\mu^n_k(t)$ is the weighted portion of workers having load $k$. Let $\mu_{\pi}^n$ denote this measure when the $n$-queue system is in equilibrium. 
By the ansatz, $\mu^n_{\pi}$ converges to a fixed limiting measure $\mu_{\pi}$ that is independent of the size of the first queue, \ie as $n\rightarrow \infty$, the background distribution $\mu_{\pi}$ is independent of queue 1. In fact, the actual arrival at queue 1 is specified by a state dependent Poisson process of rate $\lambda_K$ when the queue size is $k$. Let $M_k = \sum_{j \geq k} \mu_{\pi, j}$. One can see that 
$\lambda_k = \alpha \left(\frac{M^2_k - M^2_{k - 1}}{M_k - M_{k + 1}}\right).$ A fixed point solution is when $\mu_{\pi, k} = \alpha^{\frac{2^k - 1}{2 - 1}}$. This implies:
\vspace{-1mm}
\begin{lemma}\label{lem:loglog}Consider PPoT at the stationary distribution, with high probability, the maximum queue is in $O(\log \log n)$. 
\vspace{-6mm}
\end{lemma}


\vspace{-3mm}
\subsection{Learning the parameters}\label{sec:alearning}
\vspace{-3mm}
Wlog, assume that the average service rate of the workers is $1$. The total amount of unused compute power is $(1-\alpha)n$, where $\alpha$ is the load ratio. We further assume $\alpha$ is known because this can be easily estimated. 
\vspace{-1mm}

\myparab{Performance goal and handling excessively slow servers.} Our estimation procedure aims to efficiently estimate all $\mu_i$ within a short period but doing so is impossible for excessively slow workers, \ie waiting for one job to complete is unacceptable. Our crucial observation is that if a server's processing power is too weak, we can safely ignore it (\ie set the estimate to be $0$). Specifically, we set $\epsilon = \frac{3}{10}(1-\alpha)$ so that $(1-\epsilon)^3 \geq \frac{10\alpha}{9+\alpha}$. We need wait only for $(1+\epsilon)L/\mu$ time. If the estimation takes longer, we stop and  set the estimate to 0. 
%If estimation takes longer than that, we give up and set the estimate to $0$. 
Using standard Chernoff bound, we have:
\vspace{-2mm}
\begin{lemma}\label{lem:learn}
$\proc{Learner-aggregate}(\mbox{worker } i)$ in Fig.~\ref{fig:learner} possesses the following properties:
\emph{(i)} For any workers $i$ such that $\mu_i \leq (1-\epsilon)\frac{1-\alpha}{10}$, our estimate will be $\hat \mu_i = 0$ (\ie all slow servers will be discarded); \emph{(ii)} For any workers $i$ such that $\mu_i \geq \frac{1-\alpha}{10}$, our estimate needs to be an underestimate and guarantees $\epsilon$-multiplicative error, \ie $(1-\epsilon)\mu_i \leq \hat \mu_i \leq \mu_i$; and \emph{(iii)} For any workers $i$ such that $(1-\epsilon)\frac{1-\alpha}{10} \leq \mu_i \leq \frac{1-\alpha}{10}$, we have either $\hat \mu_i = 0$ or $(1-\epsilon)\mu_i \leq \hat \mu_i \leq \mu_im$ 
\ie it could be discarded; but if it is kept, our estimate will be reliable.  
\vspace{-2mm}
\end{lemma}
\vspace{-1mm}
\myparab{Reliable estimates imply an efficient system.} Finally, we have (see the technical report for the analysis~\cite{rosella-tr}):

%show that if the estimates satisfy the above properties, 
\vspace{-2mm}
\begin{lemma}
Consider a PPoT system in which the algorithm uses estimates $\hat \mu_i$ that satisfy the aforementioned properties. We have: (i) The PPoT process is stationary, and (ii) With high probability the maximum queue is $O(\log \log n)$ and the convergence time is $O(1)$. \label{lem:ppotgood2}
\vspace{-4mm}
\end{lemma}

==> sections/analysis_full.tex <==
\section{Analysis of the algorithms}\label{sec:analysis}
\vspace{-3mm}
\myparab{Our model.}  We consider a distributed system that consists of $n$ workers/servers, each connected to a scheduler. Jobs arriving to the scheduler may contain one or more tasks. When a new job arrives, the scheduler probe a certain number of workers and decide how 
to assign tasks based on workers' queue length. For simplicity, our theoretical model focuses on the case of one job containing one task (but our evaluation will consider the general case). 

The arrivals of jobs follows a Poisson distribution with parameter $\lambda$. Processing/compute power of the workers is heterogeneous. The service time for a job assigned to worker $i$ follows an exponential distribution with parameter $\mu_i$. 
Let $\mu = \sum_{i \leq n} \mu_i$ be \emph{the system's the total processing power}, and $\alpha = \lambda / \mu$ be the system's \emph{load ratio}. 
Both $\mu_i$ and $\lambda$ can change over time to reflect volatility in the system. %For simplicity, let the total processing power always be larger than 
$\bar \mu$, which is always larger than the job arrival rate. 

\vspace{-1mm}
\myparab{Discrete-time counterpart.} 
We use a standard way to couple our continuous time model with a discrete time model~\cite{ross2014introduction}. The discrete time model proceeds in rounds. One of the following events occurs in each round: (i) With probability $\lambda / (\lambda + \mu)$, one new job arrives, and (ii)  With probability $\mu_i / (\lambda + \mu)$, one processing event happens at worker $i$ as follows: if the worker's queue contains one or more jobs, the the oldest job is processed first. Otherwise, nothing happens. 
One round in the discrete time model corresponds to a ``jump'' event in the continuous time model. Since we have coupled models (e.g., a convergence result for one often implies a similar result for the other), our analysis can switch between them to deliver an intuitive analysis.

\vspace{-1mm}
\myparab{Main results.} Our system is highly efficient and scalable: 
\emph{Result 1. Maximum load.} With high probability the maximum queue length is $O(\log \log n)$ at the stationary distribution, generalizing existing PoT results. \emph{Result 2. Learning speed.} The time to learn \emph{all the parameters $\mu_i$} is $O\left(\frac{\log (1/n)}{(1-\alpha)^2}\right)$. Thus, when the number of workers doubles, it takes only a constant amount of additional time to learn the system. 
\emph{Result 3. Convergence time.} When the system has reliable estimates of the processing powers, it takes additional $O(1)$ time to converge to the stationary distribution. 

\iffalse
\begin{figure*}[t!]
 \includegraphics[scale=0.4]{figures/timeline.pdf}
  \centering
  \caption{
  \vspace{-.05cm}Roadmap of our theoretical analysis. At the stationary state $t_1$, the max queue length is $O(\log \log n)$ (Lemma~\ref{lem:loglog}); at time $t_2$, the system experienced a shock so that three workers changed their processing power. It takes $O(\log(1/n)$ time to re-learn the new processing power (time spent from $t_2$ to $t_3$). See Lemma~\ref{lem:learn}. At $t_3$, we learned the parameters but some queues have backlogs (the red one). It takes an additional $O(1)$ amount of time to recover (form $t_3$ to $_4$, Proposition~\ref{prop:mixing}). \color{red} Change figure}
    \label{fig:timeline}
\end{figure*}
\fi

\myparab{Interpreting the results.} 
Consider the ``life cycle'' of \sysname. 
At $t_1$, \sysname is in stationary distribution. We apply result 1: 
the maximum load at $t_1$ is $O(\log \log n)$ with high probability. At $t_2 > t_1$, the system experiences a shock (the processing power of a large number of workers get changed) and the estimates are no longer correct.
\sysname re-learns the new worker speeds. Result 2 states that the learning time is $O(\log 1/n)$. Let $t_3 = t_2 + O(\log 1/n)$ be the time the system re-learns the worker speeds. At this time, there could be backlogs during the learning (between time $t_2$ and $t_3$) since the system has been using inaccurate estimates. Result 3 states that it takes $O(1)$ time to clear up backlogs. 
%So we need to wait more time for \sysname to return to normal.

\vspace{-1mm}
\myparab{Notations.} We use $u, v$ to represent vectors, where $u_i$ ($v_i$) represents the $i$-th entry of $u$ ($v$). $\buv$ and $\bvv$ are random vectors. We refer \sysname as a PPoT process (\textbf{p}roportional sampling + PoT). We denote a PPoT process as $\{\buv(t)\}_t$. Let the stationary distribution of a PPoT be $\buv_{\pi}$. Abusing the notation, let $\{\buv_{\pi}(t)\}$ be a PPoT process that starts with stationary distribution. 
Below, we explain our analysis of the three key results. We start with result 2 because the analysis is more complex, followed by results 1 and 3.

\vspace{-3mm}
\subsection{The ``recovery time'' of the PPoT process}\label{sec:recovery}
\vspace{-3mm}
Assume that \sysname starts with an arbitrary state (\eg recently experienced a shock) and our algorithm knows the exact $\mu_i$'s, Sec.~\ref{sec:recovery} bounds the time needed for a PPoT process to converge to the stationary distribution. 

\vspace{-1mm}
\myparab{Defining recovery time.}
One way to define recovery time is the mixing time, \ie the time for the load distribution to be statistically-close to the stationary distribution, where the statistical distance between two random vectors $\bvv$ and $\buv$ is defined as 
$\|\buv - \bvv\|_{\tv} = \sum_{w} \|\Pr[\buv = w] - \Pr[\bvv = w]\|_1$. The example below shows the statistical distance is an unsuitable metrics. 
\vspace{-1mm}
\begin{example}\label{example:load}\emph{
Consider two systems whose loads are represented by $\buv$ and $\bvv$. Let $\buv_1 = 1$ and $\bvv_1 = 0$ (\ie worker 1 in $\buv$ always has 1 task while it always has 0 task in $\bvv$). The rest workers have i.i.d. distribution. Intuitively, the distributions of two systems should be close because they differ only on the first servers. But $\|\buv - \bvv\|_{\tv}$ is 1 because their supports are disjoint (coming from the fact $\buv_1$ and $\bvv_1$ never agree).
}
\vspace{-5mm}
\end{example}

We use a new metric to better capture the closeness between two systems. 
Recall that the $\ell_0$-distance two vectors is  
$\| u - v\|_0 = \frac 1 n \sum_{i = 1}^n I(u_i \neq v_i)$, where $I(\cdot)$ is an indicator function that sets to one when its argument is true. We have,

\vspace{-1mm}
\begin{definition}[$\ell_0$-distance between loads] The $\ell_0$-distance between two random vectors $\buv$ and $\bvv$, namely $\bD(\buv, \bvv)$, is at most $\epsilon$ if there is a way to couple $\buv$ and $\bvv$ such that 
$\E[\|\buv - \bvv\|_0] \leq \epsilon$.
\vspace{-2mm}
\end{definition}

This definition measures only the number of servers that have different loads in two systems. In Example~\ref{example:load}, the statistical-distance between them is $1$, but the $\ell_0$ distance is $\frac 1 n \rightarrow 0$, as $n$ grows, thus properly capturing the fact that two systems are close.  
%The $\ell_0$-distance captures the notion of ``closeness of load vectors'' well. In the previous example (in which we consider two systems such that $\bvv_1 = 1$ and $\buv_1 = 0$). While 
%Let $\buv_{\pi}(t)$ be the load vector at time $t$ of a PPoT process that starts at the stationary distribution. 
Let $\bvv(t)$ be the load vector at time $t$ of a PPoT process that starts at an arbitrary state with $C_{\max} = \|\bvv(0)\|_{\infty}$. 
\vspace{-1mm}
\begin{definition}[Recovery time] Using the notations above, the recovery time $T(\bvv, \epsilon)$ of a PPoT process that starts with $\bvv$ is 
$
T(\bvv, \epsilon) = \min_t \left\{\bD(\bvv(t), \buv_{\pi}(t)) \leq \epsilon \right\}.$
\vspace{-2mm}
\end{definition}

Intuitively, after $T(\bvv, \epsilon)$ time, only $\epsilon$-portion of the workers are inconsistent with the stationary distribution. The rest workers all recovered. We have
\vspace{-2mm}
\begin{proposition}\label{prop:mixing} Using the notations above, the recovery time $T(\bvv, \epsilon) = O(C_{\max}\log (1/\epsilon))$, \ie it \emph{does not depend} on the size $n$ of the system. 
\vspace{-2mm}
\end{proposition}

For simplicity, we assume that $\alpha$ is suitably small. Techniques developed in our analysis can be generalized for arbitrary $\alpha$. Proving Prop.~\ref{prop:mixing} consists of two major steps: 

\vspace{-1mm}
\myparab{Step 1. A conservative estimate of the stationary distribution.} Let $\{\bvv(t)\}_t$ be an arbitrary PPoT process and $f_i$ be the PDF for the marginal distribution of worker $i$ at the stationary state. The tail of $f_i$ decays with at least exponential rate (\ie $f_i(j) \leq \rho f_i(j+1)$ for some $\rho < 1$) since the PPoT algorithm is at least as good as the proportional sampling algorithm. With Markov inequality, we have:
\vspace{-2mm}
\begin{lemma}\label{lem:loadgood} Let $\epsilon$ be an arbitrary constant and $\buv_{\pi}$ be the stationary distribution. Let $\buv_{\pi, i}$ represent the $i$-th coordinate of $\buv_{\pi}$. There exists a constant $\eta$ (that depends only on $\epsilon$) such that that: $
\Pr\left[\sum_{i \leq n}I(\buv_{\pi, i} \leq \eta) \leq (1-\epsilon) n\right] \geq 1 - \epsilon.$
\end{lemma}
\vspace{-2mm}
Lemma~\ref{lem:loadgood} implies that at the stationary distribution, most workers will have constant queue length. 
We also observe that $\|\bvv(t) - \buv_{\pi}(t)\|_0$ is \emph{not} monotonically decreasing and thus it is remarkably difficult to directly track this quantity. Thus, we focus on the evolution of $\|\bvv(t) - \buv_{\pi}(t)\|_1$:
\vspace{-5mm}
\begin{lemma}\label{lem:l1monotone} Using the notations above, we have $\|\bvv(t) - \buv_{\pi}(t)\|_1 \geq \|\bvv(t) - \buv_{\pi}(t)\|_0$. Moreover, $\|\bvv(t) - \buv_{\pi}(t)\|_1$ is monotonically decreasing regardless of the initial state $\bvv(0)$.  
\vspace{-5mm}
\end{lemma}

The monotone property is a known result and can be proved by a simple combinatorial analysis. See also~\cite{bramson2012asymptotic}. 

\vspace{-1mm}
\myparab{Step 2. $\|\bvv(t) - \buv_{\pi}(t)\|_1$ shrinks quickly.} We next show that $\|\bvv(t) - \buv_{\pi}(t)\|_1$ has exponential decay. 
We need to circumvent two key challenges: \emph{(i)} The discrepancies in loads at the same workers could increase, \ie it is \emph{not true} that $|\bvv_{i}(t) - \buv_{\pi, i}(t)|\leq |\bvv_{i}(t+1) - \buv_{\pi, i}(t+1)|$. 
Therefore, we cannot focus on individual workers only. \emph{(ii)} The loads of different workers are correlated. 

Our key idea is to identify a group of events that occur sufficiently often, and when such an event occurs, $\|\bvv(t) - \buv_{\pi}(t)\|_1$ strictly decreases. 
A deletion event at time $t$ at workers $i$ is a \emph{good deletion event} if worker $i$ is empty in one of $\{\bvv(t), \buv_{\pi}(t)\}$ and non-empty in the other one. A good deletion event has no effect on, for example, $\bvv_i$ but $\buv_{\pi, i}$ is decremented by one. After the deletion, we have $\|\buv_{\pi}(t+1) - \bvv(t+1)\|_1$ is decremented by 1. The frequency of good deletion events is:
%characterized by the following lemma. 
\vspace{-2mm}
\begin{lemma}\label{lem:shrink}Using the above notations, there exists a constant $C$ such that with constant probability, 
$\|\bvv(t+C) - \buv_{\pi}(t+C)\|_1 \leq c_1 \|\buv_{\pi}(t) - \bvv(t)\|_1
$
\vspace{-3mm}
\end{lemma}

\mypara{Outline of the proof.} When the loads of workers $i$ are different in two processes, each loads perform a ``left-drifting random walk'' with a left bound $0$. With a constant probability, within $\Theta(1)$ steps, one walk will hit zero first, and 
a good deletion event will occur. We next need to count the number of workers with different loads at $t$, \ie $\|\bvv(t) - \buv_{pi}(t)\|_0$. We observe that with high probability $\|\bvv(t) - \buv_{\pi}(t)\|_0 = \Theta(\|\bvv(t) - \buv_{\pi}(t)\|_1)$. 
When we have large number of excessively long queues, $\ell_0$-norm of a vector could be much smaller than the $\ell_1$-norm. But having excessive long queue is a rare event; we can use this intuition to show that $\ell_1$-norm and $\ell_1$-norm of  $\bvv(t) - \buv_{\pi}(t)$ are in the same order. 
Lemma~\ref{lem:shrink} and the fact that $\|\bvv(t) - \buv_{\pi}(t)\|_0 = \Theta(\|\bvv(t) - \buv_{\pi}(t)\|_1)$ imply $\|\bvv(t) - \buv_{\pi}(t)\|_0$ shrinks by a constant portion in $O(1)$ time. Prop.~\ref{prop:mixing} the follows. 

\iffalse
We now calculate the recovery time. Let $k = \|\bvv(t_0) - \buv_{\pi}(t_0)\|_1 = O(C_{\max})$ for some $t_0$. Since $\|\bvv(t_0) - \buv_{\pi}(t_0)\|_1 = \Theta(\|\bvv(t_0) - \buv_{\pi}(t_0)\|_0)$, we have $\|\bvv(t_0) - \buv_{\pi}(t_0)\|_0 \geq c_1 k$ for some constant $c_1$. 
After waiting a constant amount of time (say $\Delta$), the number of good deletion events is in the order of $c_1k$. Thus, we have $\|\bvv(t_0 + \Delta) - \buv_{\pi}(t_0 + \Delta )\|_1 \leq (1-\Theta(c_1)) \|\bvv(t_0) - \buv_{\pi}(t_0)\|_1$, which implies that the $\ell_1$-distance shrinks by a constant factor. Thus, it takes $O(C_{\max}\log(1/\epsilon))$ rounds to reach a state such that $\|\bvv - \buv_{\pi}\|_1 \leq \epsilon$. This proves Proposition~\ref{prop:mixing}. 
\fi

==> sections/exp0418.tex <==
\section{Evaluation}
{\color{red} We need new evaluation}



\mypara{1. PoT (baseline).} This is the classical power-of-two-choices algorithm. 

\mypara{2. PoT$+$LB (baseline).} This algorithm integrates the classical power-of-two-choices technique and the late-binding technique~\cite{ousterhout2013sparrow}. When one job has only one task, this is identical to the algorithm used in Sparrow. Details of late binding are in~\cite{ousterhout2013sparrow}.

\mypara{3. PSS.} This is the proportional sampling scheduler in Fig.~\ref{fig:pss}. 

\mypara{4. PSS$+$PoT.} This algorithm uses both proportional sampling and power-of-two-choices techniques (see also Fig.~\ref{fig:potunscale}). 

\mypara{5. PSS$+$PoT$+$LB.} We also examine the improvement of  PSS$+$PoT by using late binding. 

{\color{red}ZL: we may also add the following variations of algorithms for comparison}

\mypara{6. PSS$+$PoT (join-the-shortest-waiting-time)} Here, instead of joining the shortest queue, the controller put the new job to a server with shortest wait time. 

\newpage 
{\color{red} These are old evaluation results.}
We use the python simulator in Sparrow~\cite{ousterhout2013sparrow} as our
platform to evaluate our new algorithms and compare them against baseline
algorithms. Unless otherwise stated, our experiments assume that each job
contains exactly one task. At the end of this section, we also present
preliminary result for the general case where each job may contain multiple
tasks.

For the case where one job contains exactly one task, we focus on the following
algorithms:


\mypara{1. PoT (baseline).} This is the classical power-of-two-choices algorithm. 

\mypara{2. PoT$+$LB (baseline).} This algorithm integrates the classical power-of-two-choices technique and the late-binding technique~\cite{ousterhout2013sparrow}. When one job has only one task, this is identical to the algorithm used in Sparrow. Details of late binding are in~\cite{ousterhout2013sparrow}.

\mypara{3. PSS.} This is the proportional sampling scheduler in Fig.~\ref{fig:pss}. 

\mypara{4. PSS$+$PoT.} This algorithm uses both proportional sampling and power-of-two-choices techniques (see also Fig.~\ref{fig:potunscale}). 

\mypara{5. PSS$+$PoT$+$LB.} We also examine the improvement of  PSS$+$PoT by using late binding. 

We do not consider the uniform algorithm because in most cases this algorithm is considerably worse than the rest of the algorithms. 

Our simulation consists of 100 servers with four cores per server. Following assumptions made in~\cite{ousterhout2013sparrow}, we do not consider the impact of network delays. 

\myparab{Heterogeneous servers.} We use parameters $\{\lambda_i\}_{i \in [n]}$ to control the processing power of the servers. The variables $\lambda_{i}$'s follow a Zipf distribution, \ie $\Pr[\lambda_i = 1/k] \propto k^{-\eta}$, where $\eta = 2$. 
 We cap the processing power of the fastest server to be at most 100 times faster than the slowest one. 
 In our setup most servers have comparable performance but a small fraction of them
 are slower (\eg loaded with background activities, in unhealthy state, or crashing
 soon). %An % effective scheduler should not let a small number of slow servers contaminate the whole system.

\myparab{Failure of baseline algorithms.} When the servers are heterogeneous, the
baselines (PoT and PoT$+$LB) may have unbounded queue length/waiting times. See Figure~\ref{sfig:sparrowdegrade}. Here, the load ($\lambda/(\sum_{i \leq n}\lambda_i)$) is 90\%. The $x$-axis represents the time elapsed since the system starts, where a unit of time is set to be $1/\lambda$. The average response times of all the baseline algorithms monotonically increase as the time elapsed increases, and they are unbounded. On the other hand, the response times of our algorithms (PSS, PSS$+$PoT, PSS$+$PoT$+$LB) stay stationary. 

\begin{figure}[t!]
 \includegraphics[scale=0.55]{figures/sparrowdegrades.pdf}
  \centering
  \caption{When load is $90\%$, the expected response time of baseline algorithms grows to infinite in the long run but our algorithms have stationary waiting time. A unit of time is $\lambda$ (arrival rate of the jobs).}
    \label{sfig:sparrowdegrade}
\end{figure}

%\Znote{TODO: 1. add uniform, 2. change $x$-axis into time, 3. change Pure PSS to PSS, and 4. Remove batch}
%Figure \ref{sfig:others} shows both the batch sampling and random sampling degrade about 13X to 1000X worse than our PSS. 
%\Znote{merge 4 and 6.}\Znote{1. Why PSS$+$LB and PSS are different? 2. Why PSS does not work?}}

%

\begin{figure}[ht!]
 \includegraphics[scale=0.55]{figures/response_time_500000.pdf}
  \centering
  \caption{Sparrow, batch, and PSS performance under different loads for the first 500k jobs. When the load is high (\eg 0.9), the baselines are not stationary so their response times will grow when there are more jobs.}
    \label{sfig:load}
\end{figure}


\myparab{Our algorithms vs. baselines.} We next compare the performance of our algorithms against the baselines after the system is warmed up (after processing 500,000 jobs). We focus on how the response times change as we vary the system's load. See Fig.~\ref{sfig:load}. Note here that we measure the average response time for \emph{finite sample size} (specifically, the first 500,000 jobs). When the load is high (\eg 0.9), the baselines are not stationary so their response times will grow when there are more jobs.

We have the following observations. $(i)$ The simple PSS already outperforms all
baseline algorithms. $(ii)$ When PoT is integrated into PSS, the performance
gain is moderate for the low load case, and is significant when the load is
close to one. $(iii)$ When we integrate late binding with PSS$+$PoT, the
performance gain is moderate.

We also observe that the baselines' response times decrease when the load from
0.1 to 0.5, while they increase when the load increases from 0.5 to 1. The
reason is that most servers are idle when the load is small. In this case, slow
servers are more likely to be chosen. When the load increases,  slow servers are
occupied so they are less likely to be chosen, leading to a decrease in response
time. Finally, as the load further grows, the system starts to be saturated so
everything slows down.

\myparab{Scaled vs. unscaled policies.} We next verify that the scaled policy under PSS$+$PoT is a better choice. We consider two scenarios. 

\mypara{1. Policies ``at the limit''.}  As discussed in Section~\ref{sec:prop},
when we are allowed to probe all servers, the scaled and unscaled policies
reduce to the shortest-queue and the shortest-response-time algorithms.
Fig.~\ref{fig:scaledgreedy} compares these two algorithms. Here, we observe that
both algorithms have the same waiting time when the load is small, and that
because the shortest-response-time algorithm chooses the faster server, its
response time is faster. We also observe that when the load approaches one, the
shortest-queue algorithm significantly outperforms the shortest-response-time
one in both waiting time and response time.

%but the shortest-queue algorithm significantly outperforms the shortest-response-time one when the load is larger than $0.8$.

%We can see that the shortest-queue-time algorithm's performance remains stable while the shortest-response-time has the dramatically increase when load is large, especially when the load larger than 0.8.


\mypara{2. Scaled vs. Unscaled policies.}  
We then examine the impact of using scaled policies for PSS$+$PoT. See Fig.~\ref{fig:scaledpot}. One can see that the performance here resembles the performance of the algorithms in Fig.~\ref{fig:scaledgreedy}, \ie the scaled policy degrades significantly as the load approaches to 1. 


%But in general, the difference is less pronounced than that shown in Fig.~\ref{fig:scaledgreedy}.




\begin{figure}
  \centering
  \begin{tabular}[b]{c}
  \hspace*{-0.3in}
    \includegraphics[width=.51\linewidth]{figures/greedy_vs_scaledgreedy.pdf} \\
    \small Response time
  \end{tabular} \qquad
  \begin{tabular}[b]{c}
  \hspace*{-.45in}
    \includegraphics[width=.51\linewidth]{figures/greedy_delay.pdf} \\
    \small Waiting time
  \end{tabular}
\caption{The impact of greedy policy. We compare the performance of shortest-response-time and shortest-queue algorithms. }
\label{fig:scaledgreedy}
\end{figure}

\iffalse
\begin{figure}[!t]
    \subfloat[Response time\label{fig:ds2pass}]{%
     \includegraphics[width=0.22\textwidth]{figures/greedy_vs_scaledgreedy.pdf}
      %\includegraphics [scale = 0.4]{figures/datadiagrams/bar_fetch.pdf}
      } 
    \hfill 
    \subfloat[Waiting time\label{fig:specds}]{%
      \includegraphics[width=0.22\textwidth]{figures/greedy_delay.pdf}
      %includegraphics [scale = 0.4]{figures/datadiagrams/bar_write.pdf}
    }
\caption{The impact of greedy policy. We compare the performance of shortest-response-time and shortest-queue algorithms. }
\label{fig:scaledgreedy}
\end{figure}



\begin{figure}[htbp]
\begin{minipage}[t]{0.5\linewidth}
\begin{subfigure}
    \includegraphics[width=\linewidth]{figures/greedy_vs_scaledgreedy.pdf}
\end{subfigure}}
\end{minipage}%
    \hfill%
\begin{minipage}[t]{0.5\linewidth}
\begin{subfigure}
    \includegraphics[width=\linewidth]{figures/greedy_vs_scaledgreedy.pdf}
    \end{subfigure}}
    \caption{waiting time}
    \label{f2}
\end{minipage} 
\end{figure}


\begin{figure}[ht!]
 \includegraphics[scale=0.5]{figures/greedy_vs_scaledgreedy.pdf}
 \includegraphics[scale=0.5]{figures/greedy_delay.pdf}
  \centering
  \caption{The impact of greedy policy. We compare the performance of shortest-response-time and shortest-queue algorithms. }
    \label{fig:scaledgreedy}
\end{figure}
\fi

\iffalse
\begin{figure}[ht!]
 \includegraphics[scale=0.5]{figures/RTload95.pdf}
 \includegraphics[scale=0.5]{figures/delay_load95.pdf}
  \centering
  \caption{The impact of greedy policy when load is 0.95
 }
    \label{fig:scaledgreedy95}
\end{figure}
\fi

\begin{figure}[ht!]
 \includegraphics[scale=0.6]{figures/PoT_PSS_scale.pdf}
  \centering
  \caption{The impact of using scaled policy in PSS$+$PoT.}
    \label{fig:scaledpot}
\end{figure}


\myparab{Multiple tasks in the same job.} We next consider the scenario in which one
job consists of multiple tasks. Here, we assume each job contains exactly 100 tasks
and the cluster contains 10,000 servers. All the algorithms use the batching trick
~\cite{ousterhout2013sparrow}. Statistics are collected after the system ``warms up''
(after 50,000 jobs). Fig.~\ref{mul} shows the result. We observe that the best four
algorithms all use PSS, with the best two being PSS$+$PoT$+$LB and PSS$+$PoT. PSS$+$PoT
has worse performance than PSS$+$PoT$+$LB when the load is close to 1. We also observe
that PSS-based algorithms are significantly better even when the load is small. More
comprehensive evaluation for the multiple-task scenario is our future work.

\iffalse
%tasks scenarios, which each job contains 100 task running on a cluster with 10000 servers. 
We fix the number of jobs as 50,000 and Fig. \ref{mul} shows our PSS algorithms remain stable with less response time.
The performance of Sparrow is further decreased when one job has multiple tasks. That is because the response time of job depends on the longest task completion time,
in another word, if one task hits the very slow server, then the response time is increased. 
\fi



\begin{figure}[ht!]
 \includegraphics[scale=0.5]{figures/mul.pdf}
  \centering
  \caption{The performance of response time when one job contains 100 tasks.}
    \label{mul}
\end{figure}


% \myparab{Experiment 6. The impact of not knowing the parameters.} Suppose we do not know $\lambda_i$. What we shall do?



\iffalse
\section{Todo: } 
Below is a todo list 
\begin{enumerate}
\item discuss what happens if there is an exponential number of tasks in each job [exponential number means the number comes from an exponential distribution]. 
\item discuss when the algorithm falls apart, when the jobs are heterogeneous. discuss that even power-of-two choices will have trouble. 
\item explain that we need to do proportional sampling. 
\item explain that scaling and no scaling with result in two different stationary states. 
\item We do not yet have discretized analysis for the continuous time load balancing. So maybe we need two steps. 
\end{enumerate}


The discretization of continuous time has not yet been explicitly discussed. 

\begin{enumerate}
\item Power of two choices fails to work in heterogeneous system. 
\item Proportional sampling 
\item Studies of scaled and non-scaled version. 
\item The impact of not knowing the parameters. 
\item The impact that one job may contains multiple tasks. 
\end{enumerate}
\fi


%, we demonstrate that the performance of Sparrow(Batch+PoT+LB) and the other uniform load-balancing methods(Batch+PoT) degrades in the heterogeneous cluster. 

%Besides that, as we stated, different servers might have different computation power. 
%We assume Zipf law \cite{zipflaw} governs the computation power distribution with the constraint that the fastest server is no more 100 times faster than the slowest server.  

\iffalse
\myparab{Experiment 1. Sparrow and other uniform load balancing algorithm does not work.}

We evaluate the average response time running from 100,000 jobs to 1,000,000 jobs(1 task per job) under the heavily loaded servers where the load(fraction non-idle workers) is set to  90\%.
As shown in Figure \ref{sfig:sparrowdegrade}, the response time of Sparrow and batch combined power-of-two-choices are increased dramatically while our PSS algorithms remain stable with the growing of job number. 
\begin{figure}[t!]
 \includegraphics[scale=0.5]{figures/sparrowdegrade2.pdf}
  \centering
  \caption{Comparison of PSS with uniform load balancing algorithms in a simulated cluster composed of 100 machines}
    \label{sfig:sparrowdegrade}
\end{figure}

Figure \ref{sfig:load} plots the response time when the number of jobs is fixed as 50,000 jobs with the load varying from 10\% to 95\%.
Despite of  increasing the load, PSS remains stable using less response time while  
both Sparrow and batch sampling have the first decrease and then increase trend.

Our algorithm is proportional sampling, and we always give the faster server larger probe probability. Thus, the PSS is robust to the change of load.


\myparab{Experiment 2. Even simple proportional algorithm (without power-of-two-choices and late binding) work.} 

We compare simple PSS with Sparrow which has late binding and power-of-two choices under a moderately loaded cluster.
We fix the cluster load at 50\% and vary the number of jobs from 100,000 to 1,000,000.

Figure \ref{PurePSS} demonstrates that even the simple proportional algorithm only consumes 80\% response time compared to Sparrow.
Meanwhile, when we leverage the power-of-two choices and late binding on simple PSS, the response time is further reduced.

\begin{figure}[ht!]
 \includegraphics[scale=0.5]{figures/purePPSisbetter.pdf}
  \centering
  \caption{Pure PSS outperforms Sparrow}
    \label{PurePSS}
\end{figure}

\myparab{Experiment 3. Power of two choices.} 

Figure \ref{pot1} demonstrates the performance gain when we leverage the power of two choices. This effect is most apparent after 80\% load.

\begin{figure}[h]
 \includegraphics[scale=0.5]{figures/pot1.pdf}
  \centering
  \caption{Performance gain using power-of-two choices}
    \label{pot1}
\end{figure}

Then we plot the scaled version, unscaled version of power-of-two-choices, simple PSS and PSS combined  power-of-two-choices in  Figure \ref{scaledpot}.
For the simple PSS, the scaled version and unscaled version has similar performance while for the others
 the unscaled version has a better performance, which is explained in Section \ref{extension_to_PoT}.
Both simple PSS and  PSS combined power-of-two-choices  provide less response time where PSS combined power-of-two-choices achieves the best performance among these schemes.


In the greedy scheme, we send a probe to every server. Unscaled scheme selects the server with the shortest queue while scaled version picks the server with the shortest computation time.
Obviously, greedy schemes sends out too many probes result in the increase of network delay.
Shown in Figure \ref{scaledgreedy}, the unscaled greedy scheme is much better than the scaled version. 

Demonstrate the scaled version of greedy is bad. Then investigate whether the scaled power-of-two-choices is closer to the greedy algorithm or the unscaled version. How does the scaled power-of-two-choices compare with proportional sampling? Also, if we have late-binding, is it closer to scaled version, unscaled version, or even both of them? 

\begin{figure}[ht!]
 \includegraphics[scale=0.58]{figures/PoTvsPSS.pdf}
  \centering
  \caption{Compare PSS with  PoT}
    \label{sfig:load}
\end{figure}

\begin{figure}[ht!]
 \includegraphics[scale=0.6]{figures/scaledpot.pdf}
  \centering
  \caption{Compare scaled PoT with PSS}
    \label{scaledpot}
\end{figure}

\fi
%\Znote{So at 0.95 load, the baseline will increase if we have 500,000 jobs?}
  %One can see that the shortest-queue algorithm consistently gives better performance. 
  %\Znote{Change the name of the curves as ``shortest-waiting-time algorithm'' and ``shortest-queue algorithm''.}
  %  \Znote{Change the name of the curves as ``shortest-waiting-time algorithm'' and ``shortest-queue algorithm''.}
\iffalse
\mypara{1. Policies ``at the limit''.} As discussed in Section~\ref{}, when we are allowed to probe all the servers, the scaled and unscaled policies reduce to the shortest-queue and the shortest-waiting-time algorithms. Fig.~\ref{fig:scaledgreedy} compares these two algorithms. We can see that the shortest-waiting-time algorithm's performance is significantly worse when the load is small, being consistent with our thereotical results (Proposition~\ref{}). But when the load approaches to 1, the performance difference diminishes. Note that Proposition~\ref{} only predicts with $\Omega(\epsilon)$ probability the response time is $\Omega(1/\lambda_1)$ but it does not rule out the possibility that with prob $1-\epsilon$, the system behaves ``normal'' so Proposition~\ref{} is not inconsistent with the experiments. Tighter theoretical analysis is left as our future work. 

\mypara{2. Scaled vs. Unscaled policies.} We then examine the impact of using scaled policies for these scheduling algorithms: ii. PoT (baseline), ii. PSS, and iii. PSS$+$PoT. Here, the way choose candidate workers remains unchanged but when we decide which candidate worker to use, we find the one with shortest waiting time. Fig.~\ref{fig:scaledpot} shows the result. One can see that the performance here resembles the performance of algorithms in Fig.~\ref{fig:scaledgreedy}, \ie unscaled policies are consistently better but the performance difference between scaled and unscaled policies diminishes as the load approaches to 1. 


for these scheduling algorithms: i. PoT (baseline), ii. PSS, and iii. PSS$+$PoT. 
Here, the way we choose candidate workers remains unchanged but when we decide which candidate worker to use, we find the one with shorter response time.  
One can see that the performance here resembles the performance of algorithms in Fig.~\ref{fig:scaledgreedy}, \ie scaled policies increases as the load approaches to 1. But in general, the difference is less pronounced than that shown in Fig.~\ref{fig:scaledgreedy}.

\fi

==> sections/exp_sigcomm.tex <==
\section{Evaluation}
We perform our experiments in AWS clusters. We run one scheduler with 30 to 100 machines, depending on the experiments. We examine \sysname for both real loads (TPC-H) and synthetic loads. Synthetic loads allow us to create extreme environment to understand the robustness of different systems. We evaluate the following systems/algorithms. 

\begin{itemize}
\item Uniform random: When a new job arrives, the scheduler uniformly chooses a backend worker. 
\item Sparrow without late-binding: The classical power-of-two-choices algorithms. 
\item Sparrow with late-binding:  The full-fledged Sparrow that integrates a so-called “late-binding” technique with POT. 
\item The scheduler for heterogeneous clusters that assumes accurate information on worker speed. 
\item Multi-arm (baseline): When a new job arrives, with $\eta$ probability, we uniformly choose a worker to serve the job. With $1- \eta$ probability, we use PSS+PoT.\footnote{No existing system directly uses this baseline but since this is an intuitive design, we need to understand its performance.}
\item \sysname with one probe (i.e., PSS+Learning): The simplified Rosella algorithm that continuously estimates worker speed and uses the estimates to run proportional sampling algorithms. 
\item \sysname (i.e., PSS+PoT+Learning): The full-fledged Rosella system.
\end{itemize}

\subsection{TPC-H Load}
The TPC-H benchmark {\color{red}CITE} is representative of ad-hoc queries that have low latency requirements . Our experiments is similar to the experiments performed in {\color{red} CITE}. To replicate the prior experiments which used now-obsolete libraries (\eg Shark and some of its dependencies) we use Spark SQL and other newer libraries. 
{\color{blue} Q: seems we are using shark+spark framework}


\myparab{Setup.} 
We evaluate our performance on TPC-H benchmark on a cluster of 31 memory-optimized EC2 instances (m2.4xlarge, with 64G memory) composed 
of 1 scheduler and 30 workers.


The TPC-H workload is submitted by Shark first. Shark complies the queries into Spark stages and waits for scheduling. 
We ported Rosella and other policies into Spark as a scheduler where regard each stage as a job.  
The stages provide heterogeneous tasks where the first stage has 33 constrained tasks(needs co-resident input data) and following stages with unconstrained tasks where have 8 tasks(read shuffled data) or 1 task(aggregation). The task duration varies from 1 milliseconds to hundreds of milliseconds. Rosella handles both constrained and unconstrained tasks.  For the 2k constrained tasks, we will schedule them to the corresponding workers where have the required input while using our policies to handle unconstrained tasks.
Scheduling the TPC-H queries takes approximately 60 minutes and we report the result of 40 minutes in the middle where 6.2k requests(30k tasks) were completed.

\mypara{Controlling worker speed.} While all EC2 instances are in the same type, we modified the executor in Spark to slow down a worker $k$ times: When a worker receives a task, it executes the task and records the execution time $T$. After completing the task, the worker holds the job task $(k – 1)T$ more time and then reports to the node monitor. The request/job response time describes the time from the request is submitted to the scheduler until the last task finishes its service. 


To evaluate the performance of Rosella, we compared the Rosella's response time to Sparrow, PoT, and Multi-arm under stable environment and volatile environment. The $\eta$ in Multi-arm is set as 0.2 in our TPC-H experiments.
\begin{figure}%[!ht]
    \subfloat[In static environments]{%
       \includegraphics[width=0.452\textwidth]{figures/staticbox.pdf}
     }
     \hfill
          \subfloat[In volatile environment.\label{subfig-1:dummy}]{%
       \includegraphics[width=0.438\textwidth]{figures/chaningSpeed.pdf}
 
     }
 \caption{Response time(in ms) for TPC-H queries with different policies, demonstrating the 5th, 25th, 50th, 75th and 95th percentiles under the load of 0.8.}
     \label{fig:withlearning}
\end{figure}

{\color{blue} Need to polish the graph and add the 95th number and add pattern? Seems all of our figures don't have the y-axis description}







\begin{figure}%[!ht]
        \subfloat[In static environments]{%
       \includegraphics[width=0.45\textwidth,height=0.15\textheight]{figures/NochangingAverage.pdf}
     }
     \hfill
       \subfloat[In volatile environment.\label{subfig-1:dummy}]{%
       \includegraphics[width=0.45\textwidth,height=0.15\textheight]{figures/averageResponsewithChaning.pdf}
     }

 \caption{Average unconstrained request response time(ms).}
     \label{fig:averageResponse}
\end{figure}
    

Figure \ref{fig:withlearning} demonstrated our Rosella's (PSS+learning, PSS+PoT+learning, and PSS+PoT+LB+learning) performance compared with Sparrow, PoT, and Multi-arm in the volatile and static environment under the load of 0.8 in both static and 
Initially, we sample worker speed form Zipf's distribution and permute the worker speeds every 2 minutes.
{\color{blue} Todo add learning chart and throughput figures
}





\iffalse
\begin{figure}%[!ht]
     \subfloat[In static environment.\label{subfig-1:dummy}]{%
       \includegraphics[width=0.23\textwidth]{figures/StaticHistogram.pdf}
     }
     \hfill
     \subfloat[ In volatile environments]{%
       \includegraphics[width=0.23\textwidth]{figures/changingHistogram.pdf}
 
     }
 \caption{The histogram of unconstrained requests.}
     \label{fig:Histrogram}
\end{figure}
\begin{enumerate}
\item Fix load and plot different policy for different tpch query (similar to Fig. 8 in Sparrow).
\item Change the load and compare response time for our policy and sparrow.
\item One figure for changing working speed
\item One figure to demonstrate our polices works well under two schedulers.
\item One figure for fake task.
\end{enumerate}
\fi
{\color{blue} We need to be able to measure learning rates.}




\newpage




==> sections/from_q.tex <==


Figure \ref{fig:withlearning} demonstrated our Rosella's (PSS+learning, PSS+PoT+learning, and PSS+PoT+LB+learning) performance compared with Sparrow, PoT, and Multi-arm in the volatile and static environment under the load of 0.8 in both static and 
Initially, we sample worker speed form Zipf's distribution and permute the worker speeds every 2 minutes.
{\color{blue} Todo add learning chart and throughput figures
}




==> sections/intro0407.tex <==
\section{Introduction}

Large-scale interactive web services and advanced AI applications are
increasingly deployed in datacenters. They need to make sophisticated decisions
at realtime, based on results from executing a massive amount of computation
tasks on thousands of servers. For example, today's search engines continuously
predict queries based on the query prefixes and refresh search results showing
on browsers, all within a few tens of milliseconds~\cite{Dean2013}. This is supported by completing enormous tiny tasks on thousands of
machines that are arranged in multiple tiers of front-ends and backend-ends in
datacenters~\cite{Yu2011}. The emerging class of advanced AI applications
(e.g., self-driving cars and robotics) based on reinforcement learning need to
perform many simulations (e.g., using Monte Carlo tree search) in strict timing
requirements to determine the next action when interacting with
physical or virtual environments~\cite{Silver2016}.

It poses significant performance challenges for task schedulers to support these
applications at scale. Specifically, task schedulers are now required to provide
high throughput as they need to schedule millions of tasks per second for these
applications~\cite{ousterhout2013sparrow}. And at the same time, the scheduling needs to be
low latency as the tasks are at millisecond level.

To make the problem more challenging, task schedulers are facing heterogeneous
environments. First, heterogeneous environments that consists of CPUs, GPUs,
FPGAs, and specialized ASICs become increasingly common. Second, background
activities, interference (between virtual machines, containers and application
processes), and failures cause massive performance fluctuations, even among
servers with the same hardware configuration.

We consider the problem of designing a high-throughput, low-latency scheduler
for heterogeneous clusters in modern datacenters. Traditional load-balancing
algorithms are inadequate because they assume the servers are uniform. In fact,
a scheduler that uses the canonical power-of-two-choices (PoT) algorithm may
result in \emph{unbounded} waiting time in the long run because it could assign
more tasks to slower servers than their processing power.

\myparab{Our contribution.} We introduce two major algorithmic techniques to
circumvent the limitation of the PoT solution. First,
we introduce the \emph{proportional sampling scheduler} that accounts for
servers' heterogeneity: upon the arrival of a new task, the scheduler chooses a
worker according to a multinomial distribution so that the probability that the
$i$-th worker is chosen is proportional to its processing power, \eg if the $i$-th
worker is five times faster than the $j$-th worker, $i$-th worker is five times
more likely to be chosen. This simple algorithm reduces worst-case unbounded
longest queue length in PoT to $O(\log n)$.

Second, we marry the proportional sampling technique with the PoT technique:
upon the arrival of a new task, we execute the proportional sampling algorithm
twice to obtain two candidate workers. Then we assign the task to the worker
with the shorter queue. This algorithm reduces the worst-case queue length from
$O(\log n)$ to $O(\log \log n)$, generalizing the standard power-of-two-choices
result.

While the generalization appears to be natural,  we face the following technical
challenge: when we need to decide which of the sampled workers to use, there are
two plausible solutions.  $(i)$ \emph{Comparison by queue length}, i.e.,
comparing the raw length of the queues and use the smaller one. $(ii)$
\emph{Comparison by expected waiting time}, i.e., considering both the queue
length and processing power of two workers and choosing the worker with the
shorter expected waiting time. For example, consider a scenario in which the
queue length of the first server is ten times longer than the second one, but
the first server is 20 times faster. The queue-length based solution would
choose the second server but the expected waiting-time based solution would
choose the second server. Our analysis shows that the queue-length based
solution is the correct generalization of PoT and that it outperforms the
expected waiting-time based solution.

We extensively evaluate our new algorithms against prior solutions, including
the PoT algorithm and those that leverage additional techniques such as late
binding~\cite{ousterhout2013sparrow}. Our experiments confirm our new algorithms
have higher throughput, shorter waiting time, and shorter longest queue length.


==> sections/introduction.tex <==
\section{Introduction}
\Znote{Xin: maybe you need to think of re-writing this paragraph...}
Compute pattern of large-scale distributed system witnessed significant evolution in recent years because in part of the following changes: 
(1) \emph{The rise of data-driven, machine-learning type applications.} The wide-spread of machine-learning driven applications results in many
more self-contained small jobs such as recognizing a piece of voice (Siri), an image (deep-learning based image search), and XXX (MAKE UP MORE EXAMPLES). (2) \emph{the move to 
micro-services}. The use of containers to host micro-services is becoming increasingly standard. These container-based architectures also encourage the usage of small jobs. We also note that these two phenomenon are inter-related, \eg container-based architecture is also suitable for the deployment of ML services. 

On the other hand, these systems are often implemented on top of cloud-providers, such as AWS and Microsoft Azure. A salient feature of these cloud services is that each server may not necessarily have uniform  processing power, for the following reasons: (1) \emph{tiered services and market-drivent pricing.} 
AWS and Azure often servers at different tiers with different rates. Furthermore, such rates sometimes are decided by an auction market (\ie people trade these servers in the market) and thus fluctuate from time to time. Becaues of such non-uniform pricing mechanism, distributed system users bid for different servers from time to time to optimize the cost. Thus, the distributed server has heterogenous servers. (2) \emph{Performance discrepencies for servers at the same tier.} Even for the servers at the same tier (have the same price), they may not give the same performance for two reasons: (a) the physical servers may be different (QUOTE AMAZON PRICING, THAT THE SAME SERVICE HAVE DIFFERENT SERVERS), (b) even the servers are in the same generation and have performance difference \Znote{Cite the paper that turns on multiple VMs and keep the one with the best performance.} 

\textbf{Sell at some point that we need low latency high-throughput load-balancer.}

\Znote{Is it possible to cite something to show that there are a lot of machine learning workloads?}


Thus, many distributed systems today need to handle small jobs of uniform size using heterogenous servers. One important question arises: 

{\quote{\emph{How do we build efficient load balancers for massive scale heterogenous servers?}}}

\myparab{Randomized-load balancers.} The design of load-balancers is a very old research problem in computer science. In the traditional setting, 
there is one load-balancer and a total number of $n$ identical machines. Jobs arrive to the load balancer in a streaming fashion. Upon the arrival of a new job, the load-balancer's goal is to decide which server to serve the new job so that in long run the system is ``healthy'' and `` efficient''. Here, the load balancing algorithm needs to be simple and consume little resources (\eg small space complexity, small communication complexity, and fast decision time.) Performance metrics we aim to optimize include 

\begin{enumerate}
\item \emph{maximum queue length.} Our goal is to minimize the most heavy workloads at the stationary state, \item \emph{expected maximium waiting time.} The goal here is to minimize the maximum expected waiting time (\Znote{be a bit more careful here. Is maximum expected waiting time the same as expected maximum waiting time?}) 
\item \emph{average expected waiting time}. Here, we want to minimize the average amount of time each job needs to wait. 
\item MORE? 
\end{enumerate}

Some of these objectives are equivalent (\eg minimizing the maximum queue length and minimizing the maximum waiting time are the same). But some objectives are incompatible, \eg (maybe?) we cannot optimize average expected waiting time and maximum queue length at the same time. 

 \Znote{Need to ask around: which metrics is eventually the most important? We need to argue or there is a ``default'' most important ones?
} 

\Znote{Make a discussions on that the above metrics are more or less equivalent for the homegenous server case but such subtle differences become pronouced when we work on heterogenous systems} 

\myparab{Prior best-known algorithms.} The first ``textbook'' algorithm is to uniformly select the next. Under the assumption that the total processing power of the system is higher than the arrival rate of the jobs (articulated below), we can see that the maximum queue length is in the order of $\Theta(\log n)$. 

The next canonical example of load-balancing algorithm is the so-called ``power-of-two-choices'' algorithm. This algorithm randomly chooses two servers and use the server with smaller weight. Here, under suitable assumptions, the maximum load reduces from $\log n$ to $\log \log n$. 

An important advantage of these algorithms is that they consume little resources, \ie constant amount of communciation and space is needed. 

When the compute power is heterogenous, however, both of these algorithms are ineffective. We use an example to illustrate the problem.

\begin{example} Consider a distributed system that consists of two servers. The processing power of the first server is ten times of the second server (we will articulate how we model fast and slow computers in Section X). When we use the ``textbook uniform algorithm'', each machine serves approximately the same number of jobs. But such load-balancing scheme is intuitively wrong because the first server is supposed to undertake ten times more jobs than the second server. 
\end{example} 

It becomes immediate that the ``generalization'' of the above algorithm is that we need to sample the servers proportional to their processing power. Let us refer to such algorithm as \emph{proportional sampling algorithm}. In the forthcoming sections, 



==> sections/model.tex <==
\section{Problem formulation}
We consider a distributed system that consists of $n$ worker, each of which is connected to a scheduler. The jobs arrive to the scheduler in a streaming fashion. Each job may contain 

Upon the arrival of a new job, the scheduler can probe a constant number of workers and then decides which worker should serve for the new job. The jobs are uniform but we assume the arrivals of jobs follow a Poisson distribution with parameter $\lambda$. Processing power of the workers is heterogeneous. For the $i$-th worker, the processing time for a job follows an exponential distribution with parameter $\lambda_i$ (\ie in a unit of time, the worker can process $1/\lambda_i$ jobs on average). For the purpose of exposition, we assume $\sum_{i \leq n}\lambda_i = 1$ but this requirement is not crucial. On the other hand, we need $\lambda < 1$ to ensure the process is stationary. 

Our goal is to design a scheduling algorithm that has simple logic and be able to effectively utilize compute resources in the system. We focus on the following three metrics. 

\mypara{Expected waiting time.} On average, the amount of time a job waits before it is executed. 

\mypara{Expected completion time.} On average, the amount of time it takes for a job to complete. 

\mypara{Worst queue length.} At any moment, the length of the longest queue. 

We shall see that expected waiting time and expected completion time are closely related (they are indeed very close when the queue responsible for the job is long. On the other hand, a bound on the worst queue length ensures that the system is robust and has no outliers from time to time. 

\myparab{Discrete-time counterpart.} 
For analysis purpose, we can ``couple'' the continuous time model with a discrete time one using the standard approach. The discrete time model proceeds in rounds. In each round, one of the following events happen 
\begin{itemize}
\item With probability $\lambda/(1+\lambda)$, one new job arrives. 
\item With probability $\lambda_i/(1+\lambda)$, one ``processing'' event happens at worker $i$. This processing event works as follows: if there are one or more jobs exist in the worker's queue, then the oldest job is processed. Otherwise, nothing happens. 
\end{itemize} 

Standard coupling argument allows us to have a bijective mapping between events in the continuous time model and those that are in the discrete time model. Thus, for example, the longest queue in the continuous model is the same as the longest queue in the discrete model. 


\section{Motivation}
\Znote{mention that we use P4 switches so that we cannot do
things like late-binding}.

In the classical setting for load balancing, we assumed $\lambda_i$ are all the same. We then can use either the classical hash-based load-balancing and the power-of-two-choices algorithm. We next walk through both algorithms. 

\myparab{Hash-function based algorithm.} In this algorithm, upon the arrival of a new job, the scheduler will uniformly choose a worker and put the job over the worker. 

Under this allocation algorithm, the state of each worker follows a Markov chain. Specifically, the Markov chain's state set is the set of non-negative integers. For each time step, the transition probability is as follows: 
\begin{itemize}
\item With probability $(n-1)/n$, the Markov chain remains unchanged. This corresponds to that the event ``hits'' other workers. 
\item With probability $1/n$, the Markov chain will decide to make a move. Conditioned on this event happens, with $1/(2-\epsilon)$ ($\approx \frac 1 2 + \frac{\epsilon}{4}$) probability the Markov chain makes a ``left-move'' (\ie the chain moves to a smaller integer if it is not zero, and stays at $0$ otherwise); with $(1-\epsilon)/(2-\epsilon)$ ($\approx \frac 1 2 - \frac{\epsilon}{4}$) probability that the Markov chain makes a ``right-move''). 
\end{itemize}

Note that in the discrete time model, the Markov chains (workers) are negatively correlated (\ie, if at one specific time step, one worker makes a move, then it implies the rest workers do not move.)

Let $p_i$ be the probabiliy that the chain is at value $i$ at the stationary distribution \Znote{We need to check the actual distribution.}. One can see that $p_i$ decays exponentially \Znote{we may need to compute the exponential decay.} This implies the lemma below.

\begin{lemma}[CITE] Consider the hash-based load balancing algorithm for a system in which $\lambda_i$'s are the same. We have
\begin{itemize}
\item The expected queue length is constant over time. Also, the expected waiting time is constant as well. 
\item With high probability the maximum queue length is $O(\log n)$. 
\end{itemize}
\end{lemma}

\myparab{Power of two choices.} The power-of-two-choices algorithm aims at reducing the maximum queue length over time. The algorithm is also quite straightforward: upon the arrival of a new job, the scheduler probes two random workers and then put the new job to the worker with lighter load. This algorithm is significantly better than the Hash-function based algorithm at the worst case. 

\begin{lemma} [CITE] Consider the power-of-two-choices algorithm for a system in which $\lambda_i$'s are the same, we have whp the largest queue length is $O(\log \log n)$. 
\end{lemma}


\iffalse
\Znote{Short queue length does not translate into short waiting time.} Notice that even the max queue length for the power of two choices algorithm is $O(\log \log n)$,  the worst waiting time can still be $O(\log n)$ (even when the queue is empty, it could still takes $O(\log n)$ time to process the job). \Znote{so maybe need to ask around why PoT is good.} 

\Znote{Note that in continuous-time model, the queues or machines are independent; but in discrete time model, there 
are some negative correlations among queues.}
\fi

\subsubsection{Failure of these algorithms in heterogeneous system} 
When the compute power of each worker is different, the above algorithms (both the uniform hashing and the power of two choices) fail to work. Below provide two examples illustrating this idea. 

\begin{example} \emph{Uniform hashing does not work.} Consider a system in which there exists 10 workers. The first 9 workers can process one job on average. The last worker can process 2 jobs. So the whole system can on average process 11 jobs in one unit of time. Let the expected number of jobs that arrive in the whole system be 10.5. So we have the processing power of the system is slightly larger than the arrival rate. Now let's see what happens if we use uniform hashing for load balancing. In this case, each of the workers receives 1.05 jobs while these servers can process one job within one time unit. This implies that the process for the regular servers is non-stationary. The length of  queues associated with these servers will be unbounded. 
\end{example}

This problem persists, even using power-of-two-choices. See below for another example. Note here our example needs to use a more skewed system. 

\begin{example} \emph{Power of two choices does not work.} Consider again a system that consists of 10 workers. The first 9 workers can process one job one average. The last worker can process 6 jobs. Let the expected number of jobs that arrive in the whole system be 14. Let us refer to the first nine servers as regular servers and the last server as the fast server. In a power-of-two-choices algorithm, 
with probability $0.9 \times 0.9$ (around 0.81), two regular workers will be selected by the load-balancing algorithm (and the job will go to the one will smaller load). Thus, with probability $0.81$, a new job will go to one of the regular servers. Thus, in one unit of time, on average there are $14 \times 0.81 = 11.34$ jobs that arrive to the collection of regular servers. On the other hand, the total processing power for the regular servers is $9$. So jobs arrive more frequently than the processing power of regular servers. Thus, in long run, the queues associated with the regular servers will ``blow up''. 
\end{example}


\iffalse


\Znote{Copy existing text to here. Also mention that one job maps to one task in this particular work.}
Let $n$ be the total number of jobs in the system. 
We start with considering a continuous time model. The arrivals of jobs follow a Poission distribution, \ie the interarrival time between two jobs follows an exponential distribution with parameter $\lambda$ (so the mean is $1/\lambda$). For each machine, the time to process a job also follows exponential distribution. Different machines have different speed so we let $\lambda_i$ be the paramter for the exponential 
random variable representing the $i$-th worker. The jobs are processed in an FIFO manner. So here $1/\lambda_i$ is the average processing time for the $i$-th worker and $\lambda_i$ is the average number of jobs a worker can process within a unit of them. 
One necessary condition for the system to be stationary (or not ``blow up'') is that the processing power should be a constant fraction larger than the arrival rate. See below for an articulation of this condition.

\myparab{Requirement on the processing power of the distributed system.} Let $\lambda_1$, $\lambda_2$, ..., $\lambda_n$, and $\lambda$ be the variables defined above, a necessary condition for the system to be stationary is 
\begin{equation}
(\lambda_1 + \lambda_2 + ... + \lambda_n) \geq (1+\epsilon) \lambda, 
\end{equation}
where $\epsilon$ is a random variable. 

\textbf{Need to define processing event and how do we couple the continuous time and discrete time process.}
Note that in case the queue of a server is empty, nothing is changed (but there will be a processing event). 
\fi

==> sections/model0416.tex <==
\section{Motivation}

\myparab{Problem formulation.} We consider a distributed system that consists of
$n$ workers. We use workers and servers interchangeably. These workers are
connected to one logical scheduler. The jobs arrive to the scheduler in a streaming
fashion. Each job may contain one or more tasks. Upon the arrival of a new job,
the scheduler can probe a certain number of workers and decide how the tasks
should be assigned to the workers based on their queue lengths. For simplicity,
our theoretical model focuses on the case where one job contains exactly one
task (but our evaluation will consider the general case).

The jobs are uniform. The arrivals of jobs follow a Poisson distribution with
parameter $\lambda$ (\ie the inter-arrival time between two jobs follows an
exponential distribution with mean $1/\lambda$). Processing power of the workers
is heterogeneous. The processing time for a job assigned to worker $i$ follows
an exponential distribution with parameter $\lambda_i$. We assume $\sum_{i \leq
n}\lambda_i = 1$ but this requirement is not crucial. On the other hand, we need
$\lambda < \sum_{i \leq n}\lambda_i = 1$ to ensure the process is stationary.

Our goal is to design a simple scheduling algorithm that optimizes one or more
of the following metrics. $(i)$ \emph{Expected waiting time}: on average, the
amount of time a job waits before it is executed. $(ii)$ \emph{Expected completion
time}: on average, the amount of time it takes for a job to complete. $(iii)$
\emph{Worst queue length}: at any moment, the length of the longest queue.

We shall see that the expected waiting time and the expected completion time are closely
related. On the other hand, a bound on the worst queue length gives a bound on
the worst case waiting time.

\myparab{Discrete-time counterpart.} 
For analysis, we  couple the continuous time model with a discrete time model
using the standard approach. The discrete time model proceeds in rounds. In each
round, one of the following events happen
\begin{itemize}
\item With probability $\lambda/(1+\lambda)$, one new job arrives. 
\item With probability $\lambda_i/(1+\lambda)$, one ``processing'' event happens at worker $i$. This processing event works as follows: if there are one or more jobs in the worker's queue, then the oldest job is processed. Otherwise, nothing happens. 
\end{itemize} 
Here, one round in the discrete time process corresponds to a ``jump'' event in
the continuous-time process. Our major results are stated in terms of the
discrete-time system and they can be translated into properties in the
continuous-time system in a straightforward manner.

\subsection{Prior algorithms and their limitation}
In the standard setting, $\lambda_i$'s are assumed to be equal. Below we
describe two widely-used load-balancing algorithms and their key properties.


\myparab{Uniform algorithm.} In this algorithm, upon the arrival of a new job, the scheduler uniformly chooses a worker and puts the job over the worker. 

Under this allocation algorithm, the state of each worker follows a Markov
chain. the Markov chain's state set is the set of non-negative integers. Let
$\epsilon = 1 - \lambda$. For each time step, the transition probability of a
worker is as follows:
\begin{itemize}
\item With probability $(n-1)/n$, the Markov chain remains unchanged, which
corresponds to that a new job arrives/is processed in another worker.

\item With probability $1/n$, the Markov chain decides to make a move.
Conditioned on this event, with probability $1/(2-\epsilon)$ ($\approx \frac 1 2
+ \frac{\epsilon}{4}$),  the Markov chain makes a ``left-move'' (\ie the chain
moves to a smaller integer if it is not zero, and stays at $0$ otherwise); with
$(1-\epsilon)/(2-\epsilon)$ ($\approx \frac 1 2 - \frac{\epsilon}{4}$)
probability that the Markov chain makes a ``right-move''.
\end{itemize}

Let $\pi_i$ be the probabiliy that the chain is at value $i$ at the stationary
distribution. One can see that $\pi_i$ decays exponentially as the random walk
has a constant left-drifting term. This implies the lemma below (see
\eg~\cite{Mitzenmacher2005}).

\begin{lemma}
Consider the uniform load balancing algorithm for a system in
which $\lambda_i$'s are the same. We have: 1. The expected queue length and the
expected waiting time are constant over time; and 2. With high probability the
maximum queue length is $O(\log n)$.
\end{lemma}

\myparab{Power of two choices.} The power-of-two-choices algorithm aims at reducing
the maximum queue length over time, and works as follows: upon the arrival of a new job, the scheduler probes two random workers and then put the new job to the worker with shorter queue length. This algorithm has improved worst-case queue length (see \eg~\cite{Mitzenmacher00thepower}):

\begin{lemma} Consider the power-of-two-choices algorithm for a system in which $\lambda_i$'s are the same, with high probability the largest queue length is $O(\log \log n)$. 
\end{lemma}


\myparab{Failures of prior algorithms.} When the compute power of each worker is different, the above algorithms fail to work. 

\mypara{Example: PoT does not work.} Consider a system that consists of ten workers.
The first nine workers can process one job on average. The last worker can
process six jobs. Let the expected number of jobs that arrive in the whole
system be 14. Let us refer to the first nine servers as regular servers and the
last server as the fast server. In a power-of-two-choices algorithm, with
probability $0.9 \times 0.9= 0.81$, two regular workers will be selected. In
this case the job will go to a regular server. Thus, with probability $0.81$,
the new job uses a regular server. Thus, in one unit of time, on average there
are $14 \times 0.81 = 11.34$ jobs that arrive at the regular servers. On the
other hand, the total processing power for the regular servers is $9$. So jobs
arrive more frequently than the processing power of regular servers. Thus, in
the long run, the queues associated with the regular servers will have unbounded
lengths (\ie ``blow up''.)





==> sections/notations.tex <==
\section*{Notations}
{\color{red}This section is for internal use.  }
\begin{itemize}
\item $n$: the number of servers. 
\item $\alpha$: the load ratio. 
\item Service time/processing power: the service time of server $i$ follows an exponential distribution of parameter $\lambda_i$. $\lambda_i$ is also referred as ``processing power'' of the servers. 
\item $\lambda$ is the processing time and $\mu$ is the service time. That seems to be standard in queuing theory. 
\item $v$: the load vector (a constant). 
\item $\bvv$: the random vector. 
\item $\buv_{\pi}$: the stationary distribution. 
\end{itemize}

\subsection*{Open issues} 
Below summarizes the questions we need to answer: 
\begin{enumerate}
\item For the power law distribution, do we have a small fraction of very powerful servers, or a small fraction of computationally very weak servers? 
\end{enumerate}

==> sections/old.tex <==

{\color{red} remember to re-visit this part.}
We evaluate our system using a cluster of XXX workers and XX schedulers, running on AWS. We first examine the performance of our system using a TPC-H workload, and extensively analyze the performance of our algorithm and other baselines. Then we will use synthetic workload to characterize the system's dependencies among key parameters. 

We compare our algorithm against the following baselines:

\mypara{1. PoT (baseline).} This is the classical power-of-two-choices algorithm. 

\mypara{2. PoT$+$LB (baseline).} This algorithm integrates the classical power-of-two-choices technique and the late-binding technique~\cite{ousterhout2013sparrow}. When one job has only one task, this is identical to the algorithm used in Sparrow. Details of late binding are in~\cite{ousterhout2013sparrow}.

\mypara{3. PSS.} This is the proportional sampling scheduler in Fig.~\ref{fig:pss}. 

\mypara{4. PSS$+$PoT.} This algorithm uses both proportional sampling and power-of-two-choices techniques (see also Fig.~\ref{fig:potunscale}). 

\mypara{5. PSS$+$PoT$+$LB.} We also examine the improvement of  PSS$+$PoT by using late binding. 

{\color{red}ZL: we may also add the following variations of algorithms for comparison}

\mypara{6. PSS$+$PoT (join-the-shortest-waiting-time)} Here, instead of joining the shortest queue, the controller put the new job to a server with shortest wait time. 


\subsection{Learning with TPC-H}
to be filled in. 


==> sections/plan.tex <==
\section*{Outline of the paper}
{\color{red}This is the plan of our paper:}
\begin{itemize}
\item Section 1. Introduction: 1.5 pages. 
\item Section 2. Model and motivation: 1.5 pages. 
\item Section 3. Overview of the algorithm: 0.5 page. 
\item Section 3.1 and 3.2. Details of the algorithms: 2 pages. 
\item Section 4. analysis: 2 pages. 
\item Section 5. implementation: 0.5 page
\item Section 6. Evaluation: 3.5 pages. 
\item Section 7. Related work and conclusion: 0.5 page. 
\end{itemize}

{\color{red}ZL: we can aim to have 15 pages in the first pass, and a number of more pages in the appendix.}

{\color{red} Plots.} On average, there should be one figure per page. We need the following figures: 
\begin{itemize}
\item Section 2: we need architecture of our system. 
\item Section 3: we need to give examples of why uniform sampling does not work; why uniform power of two choices does not work. 
\item Section 4: we need to explain why join the shortest service time does not work. 
\end{itemize}



==> sections/proportional.tex <==
\section{Proportional sampling}
\label{sec:prop}

The PoT algorithm falls short in heterogeneous environments because it fails to
recognize that slower workers should process a smaller amount of jobs. Thus, we
design a new algorithm coined ``proporitional sampling scheduler'' to fix this
issue. The algorithm works as follows. When a new job arrives, it samples a
worker to serve the job and the probability the $i$-th worker is selected is
$\lambda_i$.  See also Fig.~\ref{fig:pss} for the pseudocode.

\begin{figure}
\begin{codebox}
\Procname{$\proc{Proporotional-Sampling-Scheduler}(s_i)$}
\li \Comment $s_i$ is the $i$-th job.
\li $\cald$ be a distribution on $[n]$ and $j$ with probability $\lambda_j$. 
\li $j \gets \cald$. 
\li \Comment place the job at the $j$-th server. 
\end{codebox}
\vspace{-0.2in}
\caption{The proporitional sampling scheduler.}
\vspace{-0.1in}
\label{fig:pss}
\end{figure}

We have the following lemma. 

\begin{lemma}Consider the proportional sampling algorithm. The expected queue length is constant. Furthermore, with high probability the maximum queue length is $O(\log n)$. 
\end{lemma}


\subsection{Proportional sampling with PoT}\label{extension_to_PoT}
We may further reduce the maximmum queue length of the workers by integrating
the proportional sampling procedure with the power-of-two-choices technique: we
execute the proportional sampling algorithm twice to pick up two candidate
workers. Then the ``better'' one is chosen to serve the new job. As discussed
earlier, there are two posssible policies.

\mypara{1. Use queue length (unscaled policy).} We choose the worker with the
shorter queue to serve the new job.

\mypara{2. Use expected waiting time (scaled policy).} We choose the worker with
the shorter waiting time to serve the new job.

We call the first policy ``unscaled policy'' and the second ``scaled policy''
because the latter policy is equivalent to scaling the $i$-th queue by a factor
of $1/\lambda_i$ and picking up the worker with shorter queue after scaling.

\myparab{Is being greedy healthy?} We next compare the performance of these two
policies. We note that the scaled policy leverages two algorithmic techniques:
$(i)$ sample a small portion of workers to reduce communication overhead (in our
case, we sample two); $(ii)$ use a greedy strategy to choose the worker with minimum
waiting time. We'd like to to understand how the second technique affects the
system. For the purpose of getting intuition, we temporarily ignore the the
communication constraint, \ie we assume that the system can afford probing all
the workers upon the arrival of a new job.  Thus, we can focus on comparing the
following two algorithms that represent the unscaled/scaled policies ``at the
limit''.

\mypara{1. Shortest-queue algorithm (corresponding to unscaled policy).} In this algorithm,
we choose the worker with the shortest queue to process the new job. 

\mypara{2. Shortest-waiting-time algorithm (corresponding to scaled policy).} In this
algorithm, we choose the worker with the shortest waiting time to process the new job. 

Under the first policy, the longest queue length is $O(\log n)$ whp. We next
characterize the performance of the shortest-waiting-time algorithm. Without loss
of generality,
assume $\lambda_1 \leq \lambda_2 \leq ... \leq \lambda_n$ and $\lambda_i$ ($i
\geq 2$) is a multiple of $\lambda_1$. Also, assume that $\beta = \lambda_i /
\lambda_1$. Recall that $\sum_{i \leq n} \lambda_i = 1$ and $\epsilon =
1-\lambda$. We have the following proposition.

\begin{proposition}Consider the shortest-waiting-time algorithm. At the
stationary distribution, with probability $\Omega(\epsilon)$  the length of
queue $i$ is at least $\Omega(\beta_i)$.
\end{proposition}

While we skip the formal proof here, let us interpret the
proposition. When the $i$-th queue has length $\Omega(\beta_i)$, the expected
processing time is $\Theta(\beta_i /\lambda_i) = \Theta(1/\lambda_1)$. That
means the processing time of the new job in this server is asymptotically the
same as that of the slowest server. In other words, we have the following corollary.

\begin{corollary}In the shortest-queue algorithm, with high probability the
expected waiting time is $O(1/n)$. In the shortest-waiting-time algorithm with
at least constant probability the expected waiting time is
$\Omega(1/\lambda_1)$.
\end{corollary}
Note that $\sum_{i \leq n}\lambda_i = 1$ and $\lambda_1 \leq \lambda_j$ (for all
$j$). Thus $\lambda_1 \leq 1/n$. This implies that the worst case expected
waiting time for the shortest-waiting-time algorithm is strictly worse than that
of the shortest-queue algorithm.



\myparab{Using unscaled policy in PSS$+$PoT.} The above result suggests that the unscaled policy should be used when we integrate PSS with PoT. Fig.~\ref{fig:potunscale} presents the pseudocode for the full algorithm. 

We next characterize the behavior of this algorithm. We need more notations. We let $\mu_i(t)$ be the weighted portion of workers that have load $i$ at time $t$, \ie 
\begin{equation}
\mu_i(t) = \sum_{j \leq n}I(q_j(t) = i) \lambda_j. 
\end{equation}

Also let $\mu_{\geq i }(t) = \sum_{i' \geq i}\mu_{i'}(t)$. In the case where $\lambda_i$'s are the same (\ie the standard PoT setting), we have $\mu_i(t)n$ decays in a doubly exponential manner as $i$ grows (see \eg~\cite{Mitzenmacher00thepower}). This implies that the longest queue is in the order of $\log \log n$ with high probability. Such result can be generalized to the case where $\lambda_i$ are different. Specifically, 

\begin{proposition}\label{prop:potproportion}Let $\mu_{\geq i}(t)$ be defined above. At the stationary distribution, for sufficiently large $i$, we have
\begin{equation}
\mu_{i + 1}^2(t)  \leq c_0 \mu_{i}^3(t)
\end{equation}
for some suitable constant $c_0$. 
\end{proposition}

An immediate corollary is that the maximum queue length is $O(\log \log n)$ at stationary distribution. 

\begin{proof}[sketch of Proposition~\ref{prop:potproportion}] Without loss of generality,
we that $\lambda_i \geq \epsilon/(100n)$ because we can remove all servers with $\lambda_i < \epsilon/(100n)$ without affecting system performance (\ie setting $\lambda_i = 0$ when $\lambda_i < \epsilon/(100n)$ in the algorithm).

Let $S_{\geq i}(t)$ be the set of workers with load being at least $i$ at time $t$. Note that at the stationary distribution, $\mu_{\geq i + 1}(t) = \mu_{\geq i + 1}(t + 1)$. Below we track how $\mu_{\geq i + 1}$ evolves from $t$ to $t+ 1$. 

\mypara{Events leading to decrement of $\mu_{\geq i + 1}$.} Let $\eta =1/(2-\epsilon)$ so $\eta$ is the probability that the next event is a deletion event. With probability $\eta \lambda_j$ the queue $j$ will be decremented by one at time $t + 1$. When the deletion event happens, the expected decrement in $\mu_{\geq i + 1}$ is in the order of $\sum_{j \in S_{i+1}(t)}\lambda^2_j \geq \frac 1 2 \mu_{\geq i + 1}^2(t).$ 

\mypara{Events leading to increment of $\mu_{\geq i + 1}$.} We have $1-\eta$ is the probability that the next event is an insertion event. A necessary condition that $\mu_{\geq i + 1}$ increases is that at least one of the sampled candidates is in $S_i(t)$. Thus, an upper bound on the increment is in the order of $\mu_{\geq i}\left(\sum_{j \in S_{i}(t)} \lambda^2_j\right) \leq \mu_{\geq i}^3(t)$. 

Finally, the volume of decrement should be in the same order of increment at the stationary distribution. Thus, $ \mu_{\geq i}^3(t) =O(\mu_{\geq i + 1}^2(t)).$
\end{proof}


\begin{figure}
\begin{codebox}
\Procname{$\proc{Proporotional-PoT}(s_i)$}
\li \Comment $s_i$ is the $i$-th job.
\li \Comment $q_i$ is the length of the $i$-th element. 
\li Let $\cald$ be a distribution on $[n]$ and $j$ with probability $\lambda_j$. 
\li $j_1, j_2 \gets \cald$. 
\li $j^* = \arg \min_{j \in \{j_1, j_2\}} \{q_j\}$. 
\li \Comment place the job at the $j^*$-th server. 
\end{codebox}
\vspace{-0.2in}
\caption{Integrating power-of-two-choices technique with proportional sampling.}
\vspace{-0.1in}
\label{fig:potunscale}
\end{figure}


 
\iffalse


\mypara{Proof } Note that without loss of generality, we may assume  because we may throw away all the servers with $\lambda_i < \epsilon/(100n)$ without measurable \Znote{maybe need to change this word} impact of the system. In fact, the total computing capacity of these very slow servers is bounded by $n \cdot \epsilon/(100n)$. 

But the deletion quantity and insertion quantity should be the same so we should have $\mu_{\geq i + 1}^2 = O(\mu_{\geq i}^3)$.  

\Znote{The concentration and coupling argument actually refer to a quite complex proof. We need to put the full argument in the appendix.}
\begin{enumerate}
\item We first argue that the power-of-two-choices are strictly better than proportional sampling. 
\item Then we use some Chernoff bound arguments to show that there will be no more than $3n$ jobs in the proportional sampling algorithm.  
\end{enumerate}



the Proposition suggests with constant probability, the expected waiting time is as bad as the processing time of the slowest worker. 


 Let's think about when the scheduler decides not to place the job to the first 200 servers (the slowest group). Even when a server $s_i$ ($i \leq 200$) is empty, the expected completion time is $1/\lambda_1$. On the other hand, for any server $i$, so long as the queue length is less than $\beta_i - 1$, the expected completion time is smaller than $\beta_i / \lambda_i =1/\lambda_1$. This means that a job is put to the first 200 servers only when for all the servers $i$ ($i > 200$), their queue lengths are $\geq \beta_i - 1$. 

\Znote{I have been using servers and workers interchangably. Need to fix it in the second iteration.} 

Let's also interpret the significance of such observation. First, imagine the case when $\beta_i = \sqrt n$ (or any polynomial in $n$). If we use proportional sampling, whp the queue will never be larger than $\Theta(\log n)$. But with greedy approach, the queue can be as long as $\sqrt n$ (when the first 200 servers are not all empty). Second, at the ``equilibrium'', the system behaves like every job is executed at the slowest machine. Specifically, at equilibrium, the queue length of the $i$-th server is approximately $\beta_i - 1$. So the completion time is roughly $\beta_i / \lambda_i  = 1/\lambda_1$, which is the same as the completion time when the job is executed in the slowest server. Finally, it is not uncommon that the system visits equilibrum. Specifically, the total procesisng power of the servers $i$ ($i > 200$) is $1- 2\epsilon$ while the arrival rate of the jobs is $1-\epsilon$. This means at least $\epsilon$ portion of the jobs need to be executed in the slowest server (otherwise, the length of queues on the faster servers will explode, contradicting to the fact that this process is stationary). 
That means on average, we visits the equilibrum state every $1/\epsilon$ units of time. 

In other words, we can summarize the difference between selfish scheduling and proportional sampling as follows. 

\begin{proposition} Consider the selfish scheduling algorithm. At the stationary distribution, with probability $\Omega(\epsilon)$ that the length of queue $i$ (for $i > 200$) is at least $\beta_i - 1$. On the other hand, for the proportional scheduling algorithm, with negligible probability that the longest queue is larger than $\Theta(\log n)$. 
\end{proposition}


A natural way to extend the above algorithm is to generalize the power-of-two-choices paradigm: we use the proportional sampling algorithm to independently pick up two workers. Then we pick up the ``better'' one and put the new job over there. An issue we face here is that the ``better'' is not well-defined. More specifically, consider a scenario in which two workers are chosen for a specific job. The first worker is five times faster than the second worker. The first worker has 10 jobs while the second worker has 3 jobs. Shall we choose the first one or the second one?

\begin{itemize}
\item \emph{vanilla version}: in the vanilla version, we always use the shorter queue. So in this case, we use the second worker. 
\item \emph{scaled version}: in the scaled version, we note that the first worker is 5 times faster than the second worker. So it would actually take the first worker less time to finish the new job, despite that it has a longer queue. 
\end{itemize}

Either approach looks reasonable. The second approach specifically minimizes the job's own finishing time. The impact of selfish scheduling is a new issue in heterogeneous system. Let us consider a simplified scenario to address this issue. 

\myparab{Simplified case: selfish scheduling is better or worse?}
Let's consider a simplifed selfish load-balancing problem. We shall show that a selfish load-balancing algorithm will increase the expected waiting time for all the jobs thus degrades the whole system. 


For illustration purpose, let us consider the following specific setting: 

\begin{itemize}
\item $\lambda_1 + \lambda_2 + ... + \lambda_n = 1$. Recall that $\epsilon = 1 - \lambda$.  Furthermore, $\lambda_1 = \lambda_2 = ... = \lambda_{200} = 100\epsilon / n$. 
\item $\lambda_i > \lambda_1$ for all $i \geq 200$. Furthermore, let's assume $\lambda_i$'s ($i > 200$) are all multiples of $\lambda_1$, \ie let $\beta_i = \lambda_i /\lambda_1$ and all $\beta_i$'s are integers. 
\end{itemize}

%Consider the following algorithm: \Znote{will need to change the algorithm using clrs code}
The selfish algorithm is shown in Figure~\ref{fig:selfish}. 

\begin{figure}
\begin{codebox}
\Procname{$\proc{Selfish-scheduling}(s_i)$}
\li \Comment $s_i$ is the $i$-th job 
\li \Comment $q_i$ is the length of the $i$-th element. 
\li \For $j \gets 1$ \To $n$
\li \Comment compute expected completion time to complete the job
\li \Comment if it were placed at worker $j$.
\li \Do $w_j \gets (q_j + 1)/\lambda_i$. 
\End
\li $j^* \gets =\arg \min_j \{w_j\}.$
\li \Comment place the job at the $j^*$-th server. 
\end{codebox}
\caption{The selfish-scheduling algorithm}
\label{fig:selfish}
\end{figure}

\myparab{Key observations of selfish algorithm.} Let's think about when the scheduler decides not to place the job to the first 200 servers (the slowest group). Even when a server $s_i$ ($i \leq 200$) is empty, the expected completion time is $1/\lambda_1$. On the other hand, for any server $i$, so long as the queue length is less than $\beta_i - 1$, the expected completion time is smaller than $\beta_i / \lambda_i =1/\lambda_1$. This means that a job is put to the first 200 servers only when for all the servers $i$ ($i > 200$), their queue lengths are $\geq \beta_i - 1$. 

\Znote{I have been using servers and workers interchangably. Need to fix it in the second iteration.} 

Let's also interpret the significance of such observation. First, imagine the case when $\beta_i = \sqrt n$ (or any polynomial in $n$). If we use proportional sampling, whp the queue will never be larger than $\Theta(\log n)$. But with greedy approach, the queue can be as long as $\sqrt n$ (when the first 200 servers are not all empty). Second, at the ``equilibrium'', the system behaves like every job is executed at the slowest machine. Specifically, at equilibrium, the queue length of the $i$-th server is approximately $\beta_i - 1$. So the completion time is roughly $\beta_i / \lambda_i  = 1/\lambda_1$, which is the same as the completion time when the job is executed in the slowest server. Finally, it is not uncommon that the system visits equilibrum. Specifically, the total procesisng power of the servers $i$ ($i > 200$) is $1- 2\epsilon$ while the arrival rate of the jobs is $1-\epsilon$. This means at least $\epsilon$ portion of the jobs need to be executed in the slowest server (otherwise, the length of queues on the faster servers will explode, contradicting to the fact that this process is stationary). 
That means on average, we visits the equilibrum state every $1/\epsilon$ units of time. 

In other words, we can summarize the difference between selfish scheduling and proportional sampling as follows. 

\begin{proposition} Consider the selfish scheduling algorithm. At the stationary distribution, with probability $\Omega(\epsilon)$ that the length of queue $i$ (for $i > 200$) is at least $\beta_i - 1$. On the other hand, for the proportional scheduling algorithm, with negligible probability that the longest queue is larger than $\Theta(\log n)$. 
\end{proposition}

In our experiment section, we shall see that the scaled power-of-two choices algorithm is closer to the selfish version (which is not what we like). 


By using a standard concentration and coupling argument, we can see that whp the total number of jobs in system is $\leq 3n$. Then use a Markov inequality, we have $\mu_{\geq 30}(t) \leq 0.1$ for all $t$. When $i > 30$, $\mu_{\geq i}(t)$ decays in a doubly exponential manner. Thus, fact that $\lambda_i > \epsilon/(100n)$ and Proposition~\ref{prop:potproportion} imply that at the stationary distribution, the maximum queue length is $\Theta(\log \log (n/\epsilon))$. 

The argument for Proposition~\ref{prop:potproportion} is also quite intuitive. 
\myparab{Expected deletion count:} 
\myparab{Expected insertion count:} 

Only if both $i_1$ and $i_2$ are in $S_i(t)$ will result in an increase of $\mu_{\geq i + 1}(t+1)$. 


\fi


==> sections/residual.tex <==


\section{Older stuff}
{\color{red} This section puts older text here. }

\Znote{At some point, we need to mention the following motivating example:} We envision a resource sharing system that can take advantage of time-varying available resources in large computing cluster. In this cluster, there are high-priority jobs that need to be executed from time to time. But then these jobs will only be using a constant fraction of resources but the remaining resources often are very hard to be ``capitalized.'' For example, AWS' tiny and T instances all attempt to capitalize the residual computing power but it is not very successful. \Znote{Check the accuracy.}

Our solution then is able to leverage the residual computing power even if such resources are highly volatile. The scheduler then can dynamically learn the processing power and adjust its load balancing policy in real time. 

\Znote{Another way of pitching the story is that multiple groups may share the same physical system but they want the logic for load-balancing to be separated, \ie each of them will have their own }

{\color{red} ZL's question:} if we keep asking the workers to send its throughput to the server periodically, then the server will be able to have the best possible estimate of each of the workers. No learning methods could be more effective than that. We need to find reasons to justify that this is not the case. 

\Znote{Check server vs worker. Be consistent}



\subsection{Our contribution} 
{\color{red} text here is new.}



\begin{itemize}
\item \emph{Q1. How can the processing power can be learned efficient?} Efficient algorithms for learning the processing power of the servers are not available yet. While generic algorithms were developed {\color{red} cite stochastic graidents} to infer latent parameters of servers, these algorithms are not directly optimized for schedulers. 
\item \emph{Q2. How can the system quickly recovers from change-of-processing-powers?} The processing power of the servers could have large ``intraday'' fluctuation. When an adjacent team starts a cron job (say analyzing the most recent logs), the processing power of the servers will significantly decline. On the other hand, when the cron job is completed, these servers ``recover''. Both our scheduler and our learner need to react quickly to the change of the environment. 
\item \emph{Q3. How can we build robust policies based on the estimates of the processing power?} To construct policies from processing power estimates, we require the algorithm to be \emph{simple} (because the scheduler needs to react in real time) and \emph{robust} (because the estimations could be imprecise). 
\end{itemize}  


 

Consider using the proportional power-of-two-choices policy. We have the following observations: 

\Znote{Need to mention that if a job is hashed to two servers, then both servers are called ``candidate servers'' for the job.}

\mypara{1. The probability of choosing the 1st server as a candidate server.} For each proportional sampling procedure, with $\frac 1 2$ probability that the 1st server will be selected. Thus, the probability that the 1st server is not selected after two trials is $\frac 1 4$, \ie the probability that the first server is a candidate is $\frac 3 4$. 

\mypara{2. Decision rules when the first server is a candidate.}  Next, we explain that when the 1st server is chosen as a candidate, it is ``quite likely'' that the job will be routed to the 1st server. Specifically, let the length of the 1st server be $\ell$. Even if the other candidate server has empty load, the expected processing time is $1$. But the expected processing time for the 1st server is $(\ell+1)/\mu$. Thus, when $\ell < \mu - 1$, the policy will use the 1st server. 

\mypara{3. The system's performance is bottlenecked by the slowest server.} We next examine the dynamics of the system, based on the above two observations. Let's assume that the system starts with a ``clean state'', \ie all queues are empty. In the beginning, 75\% of jobs will choose the 1st server as a candidate server and all of them will use the 1st server before its load hits $\mu - 1$. Note that the arrival rate during this period is $9/8 \mu$ while the processing rate is $\mu$. Thus, the queue will quickly build up and hit $\mu - 1$. When the queue length of the first server reaches $\mu - 1$, it could be possible that jobs will choose the slower servers even when the fastest one becomes a candidate. But the queue length of the first server will not change much because once the length ``goes down'', it will become ``favorable'' and builds up the queue again. Thus, the length of the queue will remain at around $\mu - 1$. 

When a job arrives at a slow server, the processing time is at least 1 (\ie assuming the queue is empty). When a job arrives at a faster server, the processing time is around $(\mu - 1 + 1)/\mu$ (assuming the queue's length is $\mu - 1$), \emph{which is as slow as other slower servers}. 

In general, all the machines could behave as slow as the slowest server. 

\mypara{4. Comparing against other policies.} We shall compare the above policy against the simple proportional sampling algorithm. The qualtative conclusion will also hold for the join-the-shortest-queue policy. 

Recall that in the simple proportional sampling algorithm, 50\% of the jobs will arrive to the 1st server. The ratio between the arrival and departure rate is $\frac 3 4$. Thus, the average queue length is $\frac 4 3$ \Znote{Qiong: please check this.} The average processing time for the jobs that arrive at the 1st server is $O(1/\mu)$ instead of $1$. 
In other words, in the proportional sampling scheme, 50\% of the jobs will directly benefit from the fast server. When there are more faster servers, more jobs will directly benefit from them. On the contrary, in the join-the-shortest-service-time policy, all the servers will behave like the worst server when the arrival rate fall into a specific range. 



The uinform and PoT algorithm fails to work in heterogeneous systems because it fails to recognize that slower workers will process a smaller amount of jobs. Thus, we design a new algorithm coined ``proporitional sampling scheduler'' to fix this issue. The algorithm works as follows. When a new job arrives, it samples a worker to serve the job and the probability the $i$-th worker is selected is  $\lambda_i$.  See also Fig.~\ref{fig:pss} for the pseudocode. 



We have the following lemma. 

\begin{lemma}Consider the proportional sampling algorithm. The expected queue length is constant. Furthermore, with high probability the maximum queue length is $O(\log n)$. 
\end{lemma}



\myparab{PoT generalization: join-the-shortest-queue or join-the-shortest-service-time?} We may further reduce the maximmum queue length of the workers by integrating the proportional sampling procedure with power-of-two-choices techniques: we execute the proportional sampling algorithm twice to pick up two candidate workers. Then the ``better'' one is chosen to serve the new job. As discussed earlier, there are two posssible policies {\color{red} Cite Yi Lu}: 

\begin{enumerate}
\item The \emph{join the shortest queue} policy ($\sqq$): this policy routes the incoming job to the queue with the shorter length. 
\item The \emph{join the least loaded queue} policy ($\llp$): this policy routes the incoming job to the queue to the shorter waiting time. 
\end{enumerate}

Let us consider a concrete example. 

\begin{example}Let $i$ and $j$ be two candidate servers selected to process the next job. Server $i$'s queue length is 10 and the average processing time is 1 minute. Server $j$'s queue length is 5 and the average processing time is 3 minutes. The $\sqq$ policy will choose server $j$ while the $\llp$ policy will choose server $i$.  
\end{example}


\myparab{$\llp$ policy is unhealthy. }  
We shall see in the example below that the $\llp$ policy will make all the servers behave as slow as the slowest ones (under certain workloads). Thus, we prefer using $\sqq$ policy in our system. 


\begin{figure}
\begin{codebox}
\Procname{$\proc{Proporotional-PoT}(s_i)$}
\li \Comment $s_i$ is the $i$-th job.
\li \Comment $q_i$ is the length of the $i$-th element. 
\li Let $\cald$ be a distribution on $[n]$ so that $j$ appears with probability $\lambda_j$. 
\li $j_1, j_2 \gets \cald$. 
\li $j^* = \arg \min_{j \in \{j_1, j_2\}} \{q_j\}$. 
\li \Comment place the job at the $j^*$-th server. 
\end{codebox}
\caption{Integrating power-of-two-choices technique with proportional sampling.}
\label{fig:potunscale}
\end{figure}






Recall that $\lambda$ is the arrival rate and $\mu$ is the guaranteed total processing power. Here we assume that both of them are known. We generate new jobs for estimation purpose with rate $\frac 1 2(\mu - \lambda)$. When an estimation job is created, it will be assigned to a random server (the server will be sampled uniformly, instead of being proportional to $\mu_i$). 

At the server side, it will track the processing time of each of the last $\ell$ jobs (including both estimation and regular jobs). {\color{red} Here, $\ell$ is set to be XXXX (it should depends on $\alpha$).}

When a communication needs to happen (\eg when the controller probes the server, or when the server needs to report compute result), the server will send its estimate on its own processing power based on the compute time of its last $\ell$ jobs. 

{\color{red} See Figure XXX for the pseudo code. }
\myparab{Key theoretical results.} We will have the following key theoretical results.
\begin{enumerate}
\item The learning time does not depend on the system size. 
\item The performance is optimal. 
\end{enumerate}





\myparab{$\llp$ policy considered unhealthy. }  
Our system uses $\sqq$ policy because the $\llp$ policy will effectively make all the workers behave as slow as the slowest one. See the example below

We shall see in the example below that the $\llp$ policy will make all the servers behave as slow as the slowest ones (under certain workloads). Thus, we prefer using $\sqq$ policy in our system. 

\begin{example} \emph{Consider a system that consists of $\mu + 1$ servers, where $\mu \gg 1$ is an integer. The processing rate of the first server is $\mu$. The processing rates of other servers is 1. Thus, the total processing rate is $2\mu$, and the first server is substantially faster. The arrival rate of the jobs is $1.5\mu$.}  
\end{example}


\Znote{Need to mention that if a job is hashed to two servers, then both servers are called ``candidate servers'' for the job.}

\mypara{1. The probability of choosing the 1st server as a candidate server.} For each proportional sampling procedure, with $\frac 1 2$ probability that the 1st server will be selected. Thus, the probability that the 1st server is not selected after two trials is $\frac 1 4$, \ie the probability that the first server is a candidate is $\frac 3 4$. 

\mypara{2. Decision rules when the first server is a candidate.}  Next, we explain that when the 1st server is chosen as a candidate, it is ``quite likely'' that the job will be routed to the 1st server. Specifically, let the length of the 1st server be $\ell$. Even if the other candidate server has empty load, the expected processing time is $1$. But the expected processing time for the 1st server is $(\ell+1)/\mu$. Thus, when $\ell < \mu - 1$, the policy will use the 1st server. 

\mypara{3. The system's performance is bottlenecked by the slowest server.} We next examine the dynamics of the system, based on the above two observations. Let's assume that the system starts with a ``clean state'', \ie all queues are empty. In the beginning, 75\% of jobs will choose the 1st server as a candidate server and all of them will use the 1st server before its load hits $\mu - 1$. Note that the arrival rate during this period is $9/8 \mu$ while the processing rate is $\mu$. Thus, the queue will quickly build up and hit $\mu - 1$. When the queue length of the first server reaches $\mu - 1$, it could be possible that jobs will choose the slower servers even when the fastest one becomes a candidate. But the queue length of the first server will not change much because once the length ``goes down'', it will become ``favorable'' and builds up the queue again. Thus, the length of the queue will remain at around $\mu - 1$. 

When a job arrives at a slow server, the processing time is at least 1 (\ie assuming the queue is empty). When a job arrives at a faster server, the processing time is around $(\mu - 1 + 1)/\mu$ (assuming the queue's length is $\mu - 1$), \emph{which is as slow as other slower servers}. 

In general, all the machines could behave as slow as the slowest server. 

\mypara{4. Comparing against other policies.} We shall compare the above policy against the simple proportional sampling algorithm. The qualtative conclusion will also hold for the join-the-shortest-queue policy. 

Recall that in the simple proportional sampling algorithm, 50\% of the jobs will arrive to the 1st server. The ratio between the arrival and departure rate is $\frac 3 4$. Thus, the average queue length is $\frac 4 3$ \Znote{Qiong: please check this.} The average processing time for the jobs that arrive at the 1st server is $O(1/\mu)$ instead of $1$. 
In other words, in the proportional sampling scheme, 50\% of the jobs will directly benefit from the fast server. When there are more faster servers, more jobs will directly benefit from them. On the contrary, in the join-the-shortest-service-time policy, all the servers will behave like the worst server when the arrival rate fall into a specific range. 




\myparab{2. Proportional PoT algorithm.} This module assumes that we have reasonably accurate estimates over $\mu_i$ for all $i$ (we shall refer to our estimate as $\hat \mu_i$. Intuitively, our scheduler allocate more jobs to more powerful servers. We may further reduce the maximmum queue length of the workers by integrating the proportional sampling procedure with power-of-two-choices techniques: we execute the proportional sampling algorithm twice to pick up two candidate workers. Then the ``better'' one is chosen to serve the new job. As discussed earlier, there are two possible policies: 

\begin{enumerate}
\item \emph{Use queue length (unscaled policy).} We choose the worker with the shorter queue to serve the new job. 
\item \emph{Use expected waiting time (scaled policy).} We choose the worker with the shorter waiting time to serve the new job. 
\end{enumerate}
We call the first policy ``unscaled policy'' and the second ``scaled policy''  because the latter policy is equivalent to scaling 
the $i$-th queue by a factor of $1/\lambda_i$ and picking up the worker with shorter queue after scaling.  


{\color{blue} Bring up the question of whether to use scaled version or unscaled version.}

\myparab{3. The learning algorithm.} The goal of this component is to efficiently learn the processing power of each server. We will use residual computation power of the system to estimate servers' processing power. Specifically, recall that the arrival rate of the jobs is $\lambda$ and the ``total processing power'' is $\mu$. The gap $\mu - \lambda$ then correpsonds to the residual computation power. We will create a small subset of jobs with arrival rate that is in the order of $\Theta(\mu - \lambda)$ (say $0.5(\mu - \lambda)$). Note that after the new jobs to the system, the load ratio will still be small than 1 (a necessary condition for the system to be stationary). These jobs will be uniformly distributed to the servers. We measure the  processing time of the jobs in the servers to estimate their processing power. 

Below, we explain each of the components in details. We take a bottom-up approach. First, with the assumption that $\mu_i$ and $\lambda$ are known, we describe our scheduling algorithm (Component 2). Second, with the assumption that a lower bound of $\mu$ (minimum guaranteed processing power) and $\lambda$ are known, we estimate each $\mu_i$ (Component 3). Finally, we explain how $\lambda$ is estimated (Component 1). 

{\color{red} ZL: We have made an assumption on the minimum processing power above. The assumption could be violated. Do we need to address it? }

{\color{red} I have been using controller and system interchangably. }





\myparab{Key theoretical result.} Roughly speaking, we will have the following results: 

\begin{itemize}
\item Only $o(1)$ portion of the servers will have queue length $\geq \log \log n$. 
\item The mixing time of the PPoT process is independent to the size of the system. 
\end{itemize}

\myparab{Interpretation of the result.} The second part of the result suggests that accurate parameter estimation implies fast recovery. When the system parameter changes, the system needs two stages to recover. \emph{Stage 1.} Re-learning the parameters, \ie the controller re-learns the parameters representing servers' processing power. \emph{Stage 2.} Recovering from the non-stationary states: when the scheduler uses wrong parameters, some servers could be in non-stationary states. After the new parameters are learned, the system becomes stationary but it needs more time to ``calm down'' (reaches stationary distribution). Property two above states that the ``calm down'' time is independent to the size of the system.  




This section analyzes our algorithm. Specifically, in Section~\ref{sec:appot} , we analyze the PPoT algorithm. In Section~\ref{sec:alearning}, we analyze the parameter learning module. 

\subsection{Proportional Power-of-Two-Choices}\label{sec:appot}
This section assumes that the PPoT algorithm has precise knowledge of $\mu_i$'s and $\lambda$, and it will prove the following key properties of the algorithm:

\begin{enumerate}
\item the PPoT process is a stationary process. 
\item the mixing time of the PPoT process is independent of the system size. 
\item at the stationary distribution, let $\pi_i$ be the marginal distribution of the $i$-th server. We have: i. $\pi_i$ are all the same, regardless the server speed, and ii. $\pi_i$ decays doublly-exponentially. Specifically, let $\pi_{i,j}$ be the probability that the length of server queue $i$ is $j$. Then we have $\pi_{i, j + 1} = O(\pi^2_{i, j})$. 
\end{enumerate}

\subsubsection{The PPoT process is stationary}
We now explain that the PPoT process is stationary. We reply on a powerful result coming from the queuing theory. {\color{red} the text here heavily overlaps with the other sigcomm submission. We need to be careful. Probably will move the result to the appendix.}



{\color{red}old}
ur analysis assumes that $\lambda/\mu = c$ for a suitably small constant $c$. For exposition purpose, we do not attempt to optimize $c$. In practice, $c$ could be arbitrarily close to 1\footnote{A necessary condition for the process to be stationary is that the load ratio is 1} and the recovery time is still independent to the size of the system. 


We next outline our analysis. A complete proof is deferred to the appendix. 

\myparab{Analysis step 1. Coupling with a conservative process.} 
We now describe key properties of $\{\bvv_c(t)\}$. $\bvv_{c, i}(t) \geq \bvv_i(t)$\footnote{$\bvv_i(t)$ is the $i$-th coordinate of $\bvv(t)$; $\bvv_{c, i}(t)$ is the $i$-th coordinate of $\bvv_c(t)$.} for all $i$ and $t$. This implies the CDF of the stationary distribution of $\bvv_c$ also stochastically dominates the CDF of the stationray distribution of $\bvv_{\pi}$. For example, let $F_{i}$ ($F_{c, i}$) be the 
CDF for the marginal distribution of the server $i$ at the stationary state of $\bvv_{\pi}$ ($\bvv_c$). Then we have $F_i(j) \geq F_{c, i}(j)$ for all positive integers $j$. 

{\color{red} Also introduce the notation $f_{c, i}$ and $f_i$.}

Second, each server in the conservative process is an $M/M/1$ queue, with arrival rate being (approximately) $2\lambda_i$ (recall that $\lambda_i = \frac{\lambda \cdot \mu_i}{\mu}$) and service rate being $\mu_i$. Using our assumption that $2\lambda < \mu$, all the queues are stationary. In addition, all the queues have the same stationary distrbution. Using standard results from queuing theory, we know that $f_{c, i}(j)$ decays exponentially in $j$. Thus, $f_i(j)$ also decays exponentially. 

Finally, note that $\bvv_{c, i}$ are \emph{not} independent for different $i$. This is because when an arrival event happens, \emph{two} of the queues will change their states simultaneously. 

{\color{red}Need to mention along the way, we highlight some technical challenges.}
\mypara{Markov-inequalities to get concentration.} A technical challenge arises when the queues in the conservative process are not independent. Specifically, our recovery time analysis requires us to argue that the loads of most queues will not become worse as time passes by (\ie we do not need to handle a lot of ``bad queues'' simultaneously). If the queues in the conservative process were independent, we would be able to use standard Chernoff bounds to argue that with high probability very few servers have load $c_0 \log n$ for some constant $c_0$. 

Here, without the independence condition, our analysis needs to be more delicated. It turns out that we may carefully use Markov inequalities to argue that with probability at most $\delta$ there are $\delta$ fraction of servers that are overloaded. While the concentration is weaker, it suffices for our forthcoming analysis. 

The non-independence structure among queues in the conservative process is a recurrent technical issue we need to address throughput the analysis. We shall see that we need to rely on careful manipulation of Markov inequalities. 




The distance $\bD(\bvv(t), \buv_{\pi}(t)) = \E \|\bvv(t) - \buv_{\pi}\|_0$ is \emph{not} monotonically non-decreasing {\color{red} Provide an example.}. But we can show $\E \|\bvv(t) - \buv_{\pi}\|_1$ is monotone. 

{\color{red} where should I put this paragraph?}
Recall that $\bvv$ and $\buv_{\pi}$ are coupled in the natural way {\color{red} we should mention 
the coupling argument much earlier.} When a new job arrives, $\bvv$ and $\buv_{\pi}$ will choose the same set of candidate servers and will both use $\sqq$ policy. Note that they may still choose different servers {\color{red} give an example.} so we \emph{do not expect} $|\bvv_i(t) - \buv_{\pi, i}(t)|$ is always monotonically decreasing. Instead we can guarantee only that $\|\bvv(t) - \buv_{\pi}(t)\|_1$ is monotically non-increasing. 

In addition, we also have $\E \|\bvv(t) - \buv_{\pi}\|_1 \geq \|\bvv(t) - \buv_{\pi}\|_0$.  
Thus we can focus on bounding $\E \|\bvv(t) - \buv_{\pi}\|_1$ as a function of $t$. 

{\color{red} Maybe providing a lemma?}



A sufficient condition for a good deletion event to occur is: \emph{(i).} there is a significant number of workers that do not have the same loads in two processes (\ie $\|\buv_{\pi}(t) - \bvv(t)\|_0$ is not small compared to $\|\buv_{\pi}(t) - \bvv(t)\|_1$). \emph{(ii).} 


When workers $i$ have the same loads in two processes, their loads will co-move in a deletion event and thus the $\ell_1$-distance between $\buv_{\pi}$ and $\bvv$ will not change. We have already known that that $\|\buv_{\pi}(t) - \bvv(t)\|_1 \geq \|\buv_{\pi}(t) - \bvv(t)\|_0$. Here, we need to develop new probabilistic technique to show that  $\|\buv_{\pi}(t) - \bvv(t)\|_1 = \Theta\left( \|\buv_{\pi}(t) - \bvv(t)\|_0\right)$. ii. When two servers with the same index have different loads, it will not take long for one of their queues to be zero. When this happens, a good deletion event will follow. Now we can use results developed in step 1: the conservative process $\bvv_c$ stochastically dominates $\bvv$. But in $\bvv_c$, we have each queue being a ``left-drifting random walk'' (that has a left-bound zero). {\color{red} add figures.} Thus, with constant number of steps, a good deletion event will occur (with constant probability). 


{\color{red} Be careful of the usage of $\ell_1$-distance. Sometimes it is referred as the statistical disance. Sometimes it is referred as the $\ell_1$ distance between two load vectors. }



In what follows, we shall first show that when our system uses the above estimate, the system will be stationary, and will possess all the properties of a system that uses completely accurate estimates of $\mu_i$. Then we will show our algorithm's estimation (Figure {\color{red} X}) 





Our learning component consists of two modules: 

\mypara{Module 1. Filtering out the slow servers.} This module filters out all workers with service rate $\leq \frac{1-\alpha}{10}$. 

\mypara{Module 2. Estimation with $\epsilon$-multiplicative guarantee.} We need to provide a service rate estimate for each of the rest of the workers. The estimate needs to guarantee $\epsilon$-multiplicative error (\ie the estimator $\hat \lambda_i$ needs to satisfy that $(1-\epsilon)\lambda_i \leq \hat \lambda_i \leq (1+\epsilon)\lambda_i$). 

Module 1 is needed because when a server is slow, it will take a long time to estimate its service time (one may impact the service time is $\infty$; in this case, it is not even possible to estimate the completion time of even one job). But accurately estimating these servers is unnecessary because they are slow (so they cannot contribute much compute power). 

\myparab{Using the estimates.} Let $\mu^* = (1-\alpha)/10$ and $\epsilon$ be that $(1- \epsilon)^3 \geq \frac{10\alpha}{9+\alpha}$. When $\alpha$ is a constant, $\epsilon$ is also a constant. 

We next explain how the estimates shall be integrated with the PPoT algorithm. 
Let $S$ be the set of servers after filtering, and let $\hat \lambda_i$ be the estimate for server $i$ with $\epsilon$-multiplicative guarantee. Let $\bar \lambda_i = \hat \lambda_i/\epsilon$ when $i \in S$ and $\bar \lambda_i = 0$ for $i \notin S$. We shall use $\bar \lambda_i$ as our estimate for the servers' speed. Properties of module 1 and 2 guarantee that when $i \in S$, we have 
\begin{equation}
\frac{1-\epsilon}{1+\epsilon}\mu_i \leq \bar \mu_i \leq \mu_i. 
\end{equation}
Thus $\mu_i$ is always a lower bound on $\mu$ but it is a little smaller than $\mu$. 

\begin{lemma} Using the notation above. Consider a PPoT system in which the algorithm uses $\bar \lambda_i$ as the estimate for worker $i$'s service rate. Then the PPoT process is stationary. 
\end{lemma}

{\color{red}May need to move the full proof to appendix.}
\begin{proof}
Our analysis consists of two steps. In step 1, we shall show that this PPoT system stochastically dominates another PPoT process $\calp_2$, in which the $i$-th server's true processing rate is $\bar \lambda_i$. In step 2, we shall show that $\calp_2$ is stationary. 

\myparab{Step 1. Stochastic dominance.} Recall that $\bvv(t)$ is the load vector of the PPoT process at time $t$. Let $\bar{\bvv}(t)$ be the load vector at time $t$ in $\calp_2$. At $t = 0$, we have $\bar{\bvv}(0) = \bvv(0)$. We shall show that there exists a coupling so that $\bar{\bvv}(t) \leq \bvv(t)$. 

The coupling procedure is a natural one. The arrival process and the hash functions are identical to $\bar{\bvv}(t)$ and $\bvv(t)$. For each server $i$, define two Poisson processes $\calq^{(i)})_1$ and $\calq^{(i)}_2$ so that the rate of $\calq^{(i)})_1$ is $\hat \mu_i$ and the rate of $\calq^{(i)}_2$ is $\mu_i - \hat \mu_i$. The processing events for the $i$-th server for $\bvv_i$ and $\bar{\bvv}$ is as follows: when an event from $\calq^{(i)}_1$ arrives, then a processing event in $\bar{\bvv}_i$ occurs. When an event from $\calq^{(i)}_1 \cup \calq^{(i)}_2$ arrives, a processing event in $\bvv_i$ occurs. One can see that the processing rate for $\bvv_i$ is $\mu_i$ and the processing rate for $\bar{\bvv}_i$ is $\bar \mu_i$. Furthermore, the processing events in $\bvv_i$ is a superset of the processing events in $\bar{\bvv}_i$. We can then show by induction that under this coupling, $\bar{\bvv}_i(t) \geq \bvv_i(t)$ for all $i$ and $t$. 

{\color{red} DO I need to use $\calp_2$? Maybe I can avoid using it to reduce the number of notations.}

\myparab{Step 2. Stationary of $\calp_2$.} Here, we need to show that in $\calp_2$, the load ratio is still a constant smaller than 1. First we have $\sum_{i \in S}\mu_i = n - \sum_{i \in \bar S}\mu_i = n - \left(\frac{1-\alpha}{10}\right)n$. Second, $\sum_{i \in S}\hat \mu_i \geq (1-\epsilon)(\sum_{s\in S}\mu_i) \geq (1-\epsilon)\left(n - \left(\frac{1-\alpha}{10}\right)n\right)$. Therefore, 
$\sum_i \bar \mu_i \geq \frac{1-\epsilon}{1+\epsilon}(\sum_i \mu_i) \geq \alpha n$. The last inequality uses the way we set up $\epsilon$. 
\end{proof}

Next we investigate the following questions: 

\begin{itemize}
\item \emph{Q1.} how do we determine that a system's service rate is below $\mu^*$.
\item \emph{Q2.} how can we build estimators with multiplicative guarantee? 
\end{itemize}

Both can be done via standard estimation procedures. For completeness, we outline the analysis, specifically highlighting the fact that the learning time grows logarithmically in $n$. We start with Q2 because the analysis is more standard. Then we will move to Q1. 

\myparab{Estimation with $\epsilon$-multiplicative guarantee.} Here, our goal is to estimate the service time parameter of worker $i$. As we assumed that the service time follows an exponential distribution, our goal is essentially to estimate an exponential distribution's parameter based on independent samples of it. 

Our estimator will use $L = \Theta(\frac{1}{\epsilon^2}\log(1/\delta))$ independent samples (\ie use measurement of the last $L$ jobs), where $\delta$ is a parameter controlling the probability that our estimation fails, and is often set to be $1/n^{c}$ for some suitable constant $c$ (say $10$). 

{\color{red} Do we really want to use median-of-mean estimators?}
There are many ways to build an estimator with multiplicative-error guarantee via using Chernoff-type bounds. For example, one may directly take the average of all the $L$ samples. Here, we use the well-known median-of-mean estimator {\color{red}CITE} because the analysis is simpler. 

\mypara{Median-of-Mean estimator.} Let $s_1 = c_0 \log(1/\delta)$ and $s_2 = 1 /\epsilon^2$. We collect $s_1 s_2$ samples, and divide them into groups of uniform size. Each group consists of $s_2$ samples. For each group, we calculate the mean, and our final estimator is the median of the averages. Standard analysis gives us that each average has standard deviation $\epsilon/\lambda_i$, and the median of the averages is within the range of $(1\pm \epsilon)/\lambda_i$. So the inverse of the median has multiplicative guarantee. 

\myparab{Filtering out the slow servers.} We next filter out the slow servers. We use a thresholding decision rule: if the total processing time in worker $i$ for the last $L$ is longer than $\frac{20c_0}{\epsilon^2}\log(1/\delta)$, then worker $i$ is filtered. By using standard Chernoff bound results, we can guarantee that all the servers whose service rates that are below $\mu^*/3$ are filtered, and all the servers whose service rates that are above $\mu^*$ are kept. There is no guarantee on the servers with service rates that are between $\mu^*/3$ and $\mu$. 

{\color{red} Then mention the definition of $\epsilon$-multiplicative guarantee.} 
{\color{red}  now defining the estimator}An estimator $\hat z$ has $\epsilon$-multiplicative guarantee (with respect to $x$) if we have $(1-\epsilon) z \leq \hat z \leq (1+\epsilon)z$.  




We will argue: 
\begin{itemize}
\item we can use the unused compute power to estimate the cost of the system. 
\item 
\end{itemize}



==> sections/sleep.tex <==


\subsection{Synthetic workloads}

Next, we consider synthetic workloads. Tasks are ``sleep'' tasks (i.e., after receiving a new task, the worker will sleep for a period).  
The processing time (sleep time) of $i$-th task processed by the $j$-th worker is $\tau_i/\mu_j$, where each $\tau_i$ is independently sampled from an exponential distribution with mean 100ms. $\mu_j$ controls the speed of worker $j$. Our experiments control the evolution of $\{\mu_j\}_j$ to produce heterogeneous and volatile computing environments. 

\begin{figure}%[!ht]
%\vspace{-3mm}
     \subfloat[PoT's response time is \qquad \qquad non-stationary. \label{subfig-1:dummy}]{%
       \includegraphics[width=0.21\textwidth]{figures/unbounded_length.pdf}
     }
     \hfill
     \subfloat[Response times under  different loads\label{subfig-2:dummy}]{%
       \includegraphics[width=0.21\textwidth]{figures/different_load.pdf}
     }

     \caption{Response times with known worker speeds.}
     \label{fig:sleepload}
     \vspace{-5mm}
\end{figure}


\myparab{Heterogeneity.} We first assume the worker speeds are known, which are independently sampled from a Zipf's distribution and a small number of servers are powerful.  


\mypara{1. Significant degradation in PoT and Random.} See Figure~\ref{fig:sleepload}a. The $x$-axis represents the indices of the jobs (\ie a job with a large index means it arrives late). 
When the workload is large ($\lambda /\mu = 0.9$), the PoT baseline has unbounded queue length/waiting times. The response time for uniform random policy grows too fast and is removed from the chart. The average response time grows as more jobs arrive while the PSS or PPoT algorithms' response times stay stationary. 


\mypara{2. Benefits across all loads.} We next examine the schedulers' performance under different loads. See Figure~\ref{fig:sleepload}b. The $x$-axis represents the load ratio. The $y$-axis represents the response time. 
PPoT has the best performance across all loads. Its performance improvements are moderate when the loads are low and become significant when the loads are high. Also, the moderate performance difference between Halo and PSS suggests that Halo has a limited benefit.


\myparab{Full-fledged execution.} We next examine the setting with changes in worker speeds. We reuse the random permutation model described in Sec.~\ref{sec:exp_tpch}. Specifically, the worker speeds always come from the same set, and the speeds are randomly permuted every minute. We consider two speed sets $S_1 = \{0.2, 0.3, \dots, 1.6\}$ and $S_2 = \{0.15, 0.15, 0.15, 0.15, 0.15, 0.2, 0.3, 0.4, 0.5, 0.6, 1, 1, 1, 2, 2\}$. $S_2$ represents a more heterogeneous setting. 
The workloads are chosen arbitrarily; other workloads exhibit similar qualitative behaviors. We examined include PoT, PSS+Learning, multi-armed bandit, and \sysname.    
% (with fixed sliding window)


\mypara{Determining sliding window size.}  The sliding window used to compute worker speed needs to be dynamic (see Sec.~\ref{sec:analysis}), \eg we use short windows for small loads while using long windows for large loads. While the theoretical results suggest that a sliding window of size $c/(1-\alpha)^3$ is asymptotically optimal, in practice, this window size is too conservative. Setting it to be $c/(1-\alpha)$ achieves the best performance in practice. 
Fig.~\ref{fig:volatile_sleep} shows the result (\ie  Fig.~\ref{fig:volatile_sleep}a uses $S_1$ as the worker speed set and Fig.~\ref{fig:volatile_sleep}b uses $S_2$). We observe that \emph{(i)} \sysname has the best performance across all load ratios for both loads. When the load ratio is large, the performance gap between ours and the baselines are more pronounced. When the environment is more heterogeneous ($S_2$), the performance gap also increases. 


\begin{figure}%[!ht]
\centering
     \subfloat[Worker speeds are from $S_1$ 
     \qquad(less heterogeneous). \label{subfig-1:dummy}]{%
       \includegraphics[width=0.19\textwidth]{figures/volatile_sleep_group1.pdf}
     }\hspace{3mm}
     \subfloat[Worker speeds are from $S_2$ (more heterogeneous). \label{subfig-1:dummy}]{%
       \includegraphics[width=0.19\textwidth]{figures/volatile_sleep_group2.pdf}
     }
\caption{{Performance of schedulers when worker speed changes.}}
     \label{fig:volatile_sleep}
\end{figure}

\myparab{The impact of introducing benchmark jobs.} We disable the production of benchmark jobs, and examine different dynamic window sizes (\ie try different constants $c$ for the window sizes $c/(1-\alpha)$). 
We aim to understand whether adjusting the window size can achieve the same performance without benchmark jobs.

\begin{figure}%[!ht]
\centering
     \subfloat[The impact of benchmark jobs \qquad \qquad (using $S_1$).\label{subfig-1:dummy}]{%
       \includegraphics[width=0.2\textwidth]{figures/change_speed_group1.pdf}
     }
     \hspace{2mm}
     \subfloat[The impact of benchmark jobs\qquad \qquad (using $S_2$)\label{subfig-2:dummy}]{%
       \includegraphics[width=0.2\textwidth]{figures/change_speed_group2.pdf}
     }
 \caption{{Impact of using benchmark jobs in \sysname.}}
     \label{fig:fakejobs}
     \vspace{-7mm}
\end{figure}

We use the same setup (\ie we randomly permute two worker speed sets $S_1$ and $S_2$ every minute.).
Our baselines are PSS+PoT+Learning with different sliding window sizes. Recall that the sliding window size is $c/(1-\alpha)$. We examine  
$c = \{10, 20, 30, 40\}$ (\eg w10 refers to setting $c = 10$). See Figure~\ref{fig:fakejobs} for the result.
We observe that while having longer sliding windows improves estimation quality, it does not translate into improvement in processing time. On the other hand, using fake jobs consistently improves the response times under different loads for different worker speed sets. Similar to the above experiments, the improvement of using fake jobs becomes more pronounced when the load ratio is high, or when the worker speeds are highly heterogeneous. 

\myparab{$\sqq$ vs. $\llp$ policies.} We examine the behaviors of $\sqq$ and $\llp$. The worker speed set is $\{0.2, ..., 1.6\}$. We fix the worker speeds.
%do not change in this setting. 
We arbitrarily choose four workers with different
speeds and plot the histograms of their queue lengths (normalized by the total number of jobs). 
Fig.~\ref{fig:scaledload}a shows the result. The workers are sorted according to their speeds (\eg the fastest worker is at the top). 


\mypara{1. Stationary distribution of $\sqq$.} Fig.~\ref{fig:scaledload}a shows that when we use $\sqq$, the  distributions of queue length for workers with different speed have the same distribution.
%confirming the theoretical results in Sec.~\ref{sec:potanalysis}. 



\mypara{2. $\llp$ prefers faster workers.} 
Comparing $\sqq$ (Fig.~\ref{fig:scaledload}a) with $\llp$ (Fig.~\ref{fig:scaledload}b), we can see that $\llp$ policy has a stronger preference of using faster workers even when their queues are excessively long. For example, the queue length of the faster worker is long tailed (top of Fig.~\ref{fig:scaledload}b), and is twice as long as the same worker in $\llp$ (top of Fig.~\ref{fig:scaledload}a), whereas the slowest worker (bottom of Fig.~\ref{fig:scaledload}b) has a much shorter queue. Therefore, all workers in $\llp$ will behave as slow as the slowest worker. 

\begin{figure}
   %[!ht]
   \vspace{-2mm}
     \subfloat[\small{Using $\sqq$ policy.} ]{%
       \includegraphics[width=0.19\textwidth]{figures/unscaled_speed.pdf}
     }
     \hfill
     \subfloat[\small{Using $\llp$ policy.}]{%
       \includegraphics[width=0.19\textwidth]{figures/scaled_speed.pdf}
     } 
   
     \caption{{Distribution of queue length using $\sqq$ and $\llp$ policies. From top to bottom: faster to slower workers.}} \label{fig:scaledload}
     \vspace{-4mm}
\end{figure}



